QualDash: Adaptable Generation of Visualisation Dashboards for Healthcare Quality Improvement

Adapting dashboard design to different contexts of use is an open question in visualisation research. Dashboard designers often seek to strike a balance between dashboard adaptability and ease-of-use, and in hospitals challenges arise from the vast diversity of key metrics, data models and users involved at different organizational levels. In this design study, we present QualDash, a dashboard generation engine that allows for the dynamic configuration and deployment of visualisation dashboards for healthcare quality improvement (QI). We present a rigorous task analysis based on interviews with healthcare professionals, a co-design workshop and a series of one-on-one meetings with front line analysts. From these activities we define a metric card metaphor as a unit of visual analysis in healthcare QI, using this concept as a building block for generating highly adaptable dashboards, and leading to the design of a Metric Specification Structure (MSS). Each MSS is a JSON structure which enables dashboard authors to concisely configure unit-specific variants of a metric card, while offloading common patterns that are shared across cards to be preset by the engine. We reflect on deploying and iterating the design of QualDash in cardiology wards and pediatric intensive care units of five NHS hospitals. Finally, we report evaluation results that demonstrate the adaptability, ease-of-use and usefulness of QualDash in a real-world scenario.

==> makefile <==
# This file seems to originate from something called 'the ultimate
# latex makefile' that different authors worked on. Find original
# versions at:
# http://tadek.pietraszek.org/blog/2006/03/24/the-ultimate-latex-makefile/
# (c) by Tadeusz Pietraszek
# http://www.acoustics.hut.fi/u/mairas/UltimateLatexMakefile/ 
# (c) by Matti Airas
#
# This file has been assembled and adjusted by Steven Bergner, Nov 2005
#  - support for multiple sub-texfiles
#  - fixed '=' '#' problem in mingw/msys environment (see E variable)
#  - PS compilation uses VGTC recommended settings
#  - targets restructured to make PDF by default
#
# Call 'make dvi' for minimal compilation, to check for proper latex
# syntax. This can be much faster than a full PDF generation when big
# figures are involved.
#
# Call 'make pdf' for direct compilation to PDF using pdfTeX. Note that this
# requires you to use .pdf files. pdfTeX can not use .ps or .eps graphics.
# use epstopdf to convert such files to .pdf files.
#
#----------------------------------------------------------------------------
#adjust the following for your purpose

#set the a .dvi name that corresponds to your main .tex file
DVIFILES = template.dvi
MAINTEXFILE = $(DVIFILES:.dvi=.tex)
SUBTEXFILES = 
BIBFILES = template.bib

#switch = to # when using ps2pdf in win32 (mingw/msys), i.e. uncomment 2nd line
#E=\=
E=\#

#adjust paper size: letter/a4
PAPERSIZE=letter
PDFLATEXPAPERSIZE="-sPAPERSIZE$E$(PAPERSIZE)"
DVIPSPAPERSIZE=-t $(PAPERSIZE)
#uncomment the following two lines when using option tvcgpapersize
#DVIPSPAPERSIZE=-T 7.875in,10.75in
#PDFLATEXPAPERSIZE=

#----------------------------------------------------------------------------
LATEX = latex
BIBTEX = bibtex
L2H = latex2html
PDFLATEX = ps2pdf
PDFTEX = pdflatex
DVIPS = dvips 

RERUN = "(There were undefined references|Rerun to get (cross-references|the bars) right)"
RERUNBIB = "No file.*\.bbl|Citation.*undefined" 

PSFILES  = $(DVIFILES:.dvi=.ps) 

PDFFILES7 = $(DVIFILES:.dvi=.pdf7) 
PDFFILES8 = $(DVIFILES:.dvi=.pdf8) 

PDFTEXFILES = $(DVIFILES:.dvi=.pdftex)

COPY = if test -r $*.toc; then cp $*.toc $*.toc.bak; fi 
#RM = /usr/bin/rm -f 
RM = rm -f 

all:	msg gs8

msg:
	@echo "  This script defaults to GhostScript 8.  If you are using GhostScipt 7 please type"
	@echo "  make gs7 instead.  If unsure type gs -v from the command line"
	@echo "  To use pdflatex/pdftex, type make pdf"
	@echo ""


pdf:     clean pdftex 

gs7:        clean dvi ps pdf7

gs8:        clean dvi ps pdf8

dvi:           $(DVIFILES)

ps:           $(PSFILES)

pdf7:           $(PDFFILES7)

pdf8:           $(PDFFILES8)

pdftex:         $(PDFTEXFILES)

$(MAINTEXFILE) : $(SUBTEXFILES) $(BIBFILES)

%.dvi:			%.tex
				$(COPY);$(LATEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(LATEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.pdftex:			%.tex
				echo "wir sind da"
				$(COPY);$(PDFTEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(PDFTEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.ps:			%.dvi
#				dvips -T 7.875in,10.75in -Ppdf -G0 $< -o $@  #use tvcgpapersize
#				dvips -Ppdf -G0 $< -o $@
				dvips $(DVIPSPAPERSIZE) -Pdownload35 -Ppdf -G0 $< -o $@
#				dvips $< -o $@


%.pdf7:			%.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dMaxSubsetPct$E100" \
	"-dCompatibilityLevel$E1.3" \
	"-dSubsetFonts$Etrue" \
	"-dEmbedAllFonts$Etrue" \
	"-dAutoFilterColorImages$Efalse" \
	"-dAutoFilterGrayImages$Efalse" \
	"-dColorImageFilter$E/FlateEncode" \
	"-dGrayImageFilter$E/FlateEncode" \
	"-dMonoImageFilter$E/FlateEncode" \
	$< template.pdf

#				$(PDFLATEX) $<

%.pdf8:                 %.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dPDFSETTINGS=/prepress" \
	"-dCompatibilityLevel=1.3" \
	"-dAutoFilterColorImages=false" \
	"-dAutoFilterGrayImages=false" \
	"-dColorImageFilter=/FlateEncode" \
	"-dGrayImageFilter=/FlateEncode" \
	"-dMonoImageFilter=/FlateEncode" \
	"-dDownsampleGrayImages=false" \
	"-dDownsampleColorImages=false" \
	$< template.pdf
#                               $(PDFLATEX) $<

# cleans anything that can be re-generated automatically, plus emacs backups
clean: 
				rm -f *.aux *.log *.bbl *.blg *.brf *.cb *.ind *.idx *.ilg	\
				*.inx *.toc *.out $(DVIFILES) $(PSFILES) template.pdf *~

.PHONY : all pdf ps dvi clean $(MAINTEXFILE)


==> table_figure.tex <==

\begin{table}[tb]
  \caption{VIS/VisWeek accepted/presented papers: 1990--2016.}
  \label{tab:vis_papers}
  \scriptsize%
	\centering%
  \begin{tabu}{%
	r%
	*{7}{c}%
	*{2}{r}%
	}
  \toprule
   year & \rotatebox{90}{Vis/SciVis} &   \rotatebox{90}{SciVis conf} &   \rotatebox{90}{InfoVis} &   \rotatebox{90}{VAST} &   \rotatebox{90}{VAST conf} &   \rotatebox{90}{TVCG @ VIS} &   \rotatebox{90}{CG\&A @ VIS} &   \rotatebox{90}{VIS/VisWeek} \rotatebox{90}{incl. TVCG/CG\&A}   &   \rotatebox{90}{VIS/VisWeek} \rotatebox{90}{w/o TVCG/CG\&A}   \\
  \midrule
	2016 & 30 &   & 37 & 33 & 15 & 23 & 10 & 148 & 115 \\
  2015 & 33 & 9 & 38 & 33 & 14 & 17 & 15 & 159 & 127 \\
  2014 & 34 &   & 45 & 33 & 21 & 20 &   & 153 & 133 \\
  2013 & 31 &   & 38 & 32 &   & 20 &   & 121 & 101 \\
  2012 & 42 &   & 44 & 30 &   & 23 &   & 139 & 116 \\
  2011 & 49 &   & 44 & 26 &   & 20 &   & 139 & 119 \\
  2010 & 48 &   & 35 & 26 &   &   &   & 109 & 109 \\
  2009 & 54 &   & 37 & 26 &   &   &   & 117 & 117 \\
  2008 & 50 &   & 28 & 21 &   &   &   & 99 & 99 \\
  2007 & 56 &   & 27 & 24 &   &   &   & 107 & 107 \\
  2006 & 63 &   & 24 & 26 &   &   &   & 113 & 113 \\
  2005 & 88 &   & 31 &   &   &   &   & 119 & 119 \\
  2004 & 70 &   & 27 &   &   &   &   & 97 & 97 \\
  2003 & 74 &   & 29 &   &   &   &   & 103 & 103 \\
  2002 & 78 &   & 23 &   &   &   &   & 101 & 101 \\
  2001 & 74 &   & 22 &   &   &   &   & 96 & 96 \\
  2000 & 73 &   & 20 &   &   &   &   & 93 & 93 \\
  1999 & 69 &   & 19 &   &   &   &   & 88 & 88 \\
  1998 & 72 &   & 18 &   &   &   &   & 90 & 90 \\
  1997 & 72 &   & 16 &   &   &   &   & 88 & 88 \\
  1996 & 65 &   & 12 &   &   &   &   & 77 & 77 \\
  1995 & 56 &   & 18 &   &   &   &   & 74 & 74 \\
  1994 & 53 &   &   &   &   &   &   & 53 & 53 \\
  1993 & 55 &   &   &   &   &   &   & 55 & 55 \\
  1992 & 53 &   &   &   &   &   &   & 53 & 53 \\
  1991 & 50 &   &   &   &   &   &   & 50 & 50 \\
  1990 & 53 &   &   &   &   &   &   & 53 & 53 \\
  \midrule
  \textbf{sum} & \textbf{1545} & \textbf{9} & \textbf{632} & \textbf{310} & \textbf{50} & \textbf{123} & \textbf{25} & \textbf{2694} & \textbf{2546} \\
  \bottomrule
  \end{tabu}%
\end{table}


\begin{figure}[tb]
 \centering % avoid the use of \begin{center}...\end{center} and use \centering instead (more compact)
 \includegraphics[width=\columnwidth]{paper-count-w-2015-new}
 \caption{A visualization of the 1990--2015 data from \autoref{tab:vis_papers}. The image is from \cite{Isenberg:2017:VMC} and is in the public domain.}
 \label{fig:sample}
\end{figure}

==> tex/02_rel.tex <==

%\textcolor{green}{READY FOR COMMENTS}

The structure of this section reflects TASHA's foundations in visualization task analysis as well as our focus on the use of dashboards in the healthcare sector.
% We motivate the different workflow steps in light of related work in this Section and then offer a breakdown of the TASHA workflow stages in Section~\ref{sec:overview}.

\subsection{Visualization Task Analysis}
% First define a task
The nested model for visualization design defines abstract tasks as domain- and interface-agnostic operations performed by users~\cite{Munzner2009}. 
This concept helps visualization researchers to \textit{``reason about similarities and differences between tasks''}~\cite{munzner2014visualization}. 
% Then define taxonomies and typologies
A task \textit{taxonomy} uses empirical evidence to classify tasks, whereas a \textit{typology} performs the classification on a conceptual basis.
Additionally, a \textit{task space} is a design space~\cite{jones2008teaching} that aims to consolidate taxonomies and typologies as a means to reason about all the possible ways  that tasks may manifest~\cite{schulz2013design}.
Several task taxonomies, typologies, and spaces have been introduced in the literature with the aim of mapping loosely-defined domain-specific tasks into a set of generalizable abstract tasks that can guide visualization design and evaluation~\cite{andrienko2006exploratory, meyer2015nested,brehmer2013multi, amar1,kerracher2017constructing, ahn2014task,schulz2013design}.

These classifications are intended to be used in the requirements analysis and design phases of visualization projects.
For instance, Wehrend and Lewis introduced a catalog that maps a classification of objects and operations to visualization techniques~\cite{wehrend1990problem}, while
%Amar et al. and of abstract visualization questions~\cite{amar1, amar2}.
Amar and Stasko~\cite{amar1} and Sediq and Parsons~\cite{sedig2013interaction} promoted the benefits of  typologies as a systematic basis for thinking about design.
%bridge the communication gap for task understanding, data abstraction and technique design, 
Heer and Shneiderman~\cite{heer2012interactive} used them as constructs when considering alternative data and view specification, manipulation, and analysis.
More recently, Kerracher and Kennedy~\cite{kerracher2017constructing} promoted the usefulness of these classifications as ``checklists'' of items to consider.
%Task spaces
%Jones et al. explain a design space as ``\textit{the world of all possible forms that can be generated as a combination of the dimensions of the space in response to a given design context, spanning all degrees of feasibility and practicality}''~\cite{jones2008teaching}.
By using a task space in the generative phase of design, 
 Ahn et al.~\cite{ahn2014task} identified previously unconsidered tasks in network evolution analysis.
 %requirements analysis. 

%adapting their space to user tasks requires users to express tasks in a somewhat abstract manner (e.g. \textit{``compare two variable distributions''}). We cannot make this assumption about the vast diversity of dashboard users in healthcare. Additionally, in order to position a task along Schulz et al.'s design space one must elicit some context around each task 
%Collectively, the wealth of typologies and task spaces in the literature allows visualization researchers to ground their design decisions in theory and reason about requirements for visualization software.
In this paper, we reflect on the strengths and opportunities that these task classifications offer in the context of dashboard design in healthcare. 
In deciding upon which classification to adopt, we excluded ones which require an early understanding of context and current practices for individual tasks.
For instance, Schulz et al.'s design space~\cite{schulz2013design} defines a task as a combination of five components:
$(goal$, $means$, $characteristics$, $target$, $cardinality)$.
However, understanding task $means$ was not feasible in our case due to the large and heterogeneous set of tasks we encountered.
We therefore sought a model that enables us to reduce the task space by grouping together similar tasks. We also sought a model that would allow us to reason about their naturally-expressed requirements of users. 
The TASHA workflow therefore draws from two existing task typologies: one proposed by Andrienko and Andrienko ~\cite{andrienko2006exploratory} and a second proposed by Brehmer and Munzner~\cite{brehmer2013multi}. 
The TASHA workflow makes use of the former to cluster and sub-sample the task space (Section~\ref{sec:tschar}) and the latter to guide the sequencing of tasks in a co-design setting (Section~\ref{sec:sampling}). 

\bpstart{The Andrienko \& Andrienko typology}
The Andrienko \& Andrienko typology structures data into two parts~\cite{andrienko2006exploratory}:
 \textbf{references} $\{\mathbf{R}\}$  define the contexts in which data is collected (e.g., time, space, etc.); %, for which a single \textbf{reference} represents a value combination assigned to referrential components; 
 and \textbf{ characteristics} $\{\mathbf{C}\}$, which are data attributes or measurements taken within the context defined by $\{\mathbf{R}\}$.
 A \textbf{relation} $\mathbf{\lambda}$ is a function that connects between elements of $\{\mathbf{R}\}$ and $\{\mathbf{C}\}$ to support comparisons, whereas a \textbf{pattern} $\mathbf{P(R)}$ is a configuration of the values in $\{\mathbf{C}\}$ across the set $\{\mathbf{R}\}$ or a subset of it. 
 
 %or between sets of references or characteristics/behaviours. 
%The types or referrers defined by the AA model are: \textit{time}, \textit{space}, and \textit{population}.
%The types of relations defined for these referrers include (but are not limited to):\textit{equality},  \textit{order}, \textit{distance}, \textit{ratio}, \textit{direction in space}, \textit{inclusion or subset overlap}, \textit{adjacency} and \textit{continuity}.
Tasks are classified along two main dimensions:
% Namely, they describe three \textit{task categories}: \textbf{lookup} tasks involve no relations, \textbf{comparison} tasks seek to find the relation between given model components (references/ characteristics), and \textbf{relation-seeking} tasks search for components (references/ characteristics) that exhibit a given type of relation. 
 \textit{(i)} \textit{Granularity}  distinguishes tasks that 
 involve individual references  (i.e., \textit{elementary}) from tasks that regard (sub)sets of references as a whole  (i.e., \textit{synoptic}). 
 \textit{(ii)} The  \textit{data function} dimension permutes different components of the data model for task input and output.
 For example, a task that is given a reference as input (e.g., a specific time) and asks about a measurement at that reference (e.g., a stock price) is classified as an \textit{elementary direct lookup} task. 
 The \textit{synoptic} version of the same task would enquire about a pattern (e.g., a peak) over the entire set of references (e.g., the entire time period in the data) or a subset of it (e.g., a week). 
%  We describe other AA task classes in our supplementary material. 
 %Specifically, they argue that if a set of referrers is regarded as a whole, then the task classifies as a synoptic task. 
 %At the synoptic level, rather than considering individual characteristics, a configuration of such characteristics across the entire set of referrers is of primary interest. 
% Tasks which perform a direct lookup of patterns over a known reference set are called \textbf{Behaviour Characterization (BC)} tasks; whereas tasks requiring the identification of reference subsets based on a given configuration are called \textbf{Pattern Search (PS)} tasks. 
%  Additionally, \textbf{comparison} and \textbf{relation-seeking} tasks involve relations as either outputs or inputs to the task, respectively. 

This approach offers a starting point for extensions that make formal task definitions possible (e.g.,~\cite{lammarsch2012developing}). 
It also offers a data-centric view of tasks which enables us to locate tasks pertaining to similar metrics and thereby call for visualizations of similar data constructs. 
%This can further enable the specification of which of the many variables available in NCA data should be shown on a dashboard and when. 
 
%Extensions to the AATT
%while and Lammarsch et al.~\cite{lammarsch2012developing} advocated their use as a ``checklist'' of design items to consider. 


\bpstart{The Brehmer \& Munzner typology}
Brehmer and Munzner's multi-level typology~\cite{brehmer2013multi} distinguishes three dimensions describing \textit{why} the task is performed,
\textit{how} the task is supported in terms of visual encoding, interaction and view coordination design choices, and finally \textit{what} the inputs and outputs of the task are, which allows for a characterization of tasks in sequence. 

%This is a very intuitive anatomical perspective of tasks. 
%In this intuitive anatomical perspective, tasks are described as highly granular abstract  ``actions'', such as \textit{select}, \textit{encode}, \textit{navigate}, etc. 
%This action-based description can map well-defined user tasks to visualization and interaction features design. For example,

\subsection{Dashboards in Healthcare} 
\label{sub:rel_dash}
Dashboards are broadly defined as \textit{``a visual display of data used to monitor conditions and/or
facilitate understanding''} ~\cite{wexler2017big}.
Sarikaya et al. highlighted the variety of definitions that exist for dashboards%and tensions between different genres (e.g. visual versus functional dashboard genres)
~\cite{sarikaya2019we}, while Few highlighted the disparity of information that dashboard users typically need to monitor~\cite{few2006common}.

In this paper, we focus our attention to the definition and use of visualization dashboards in a healthcare context, where Dowding et al. %adopted the definition of a dashboard as a tool \textit{``tosummarize and integrate key performance information across an organization into a visualdisplay as a way of informing operational decision making''} .
 distinguished two main categories of dashboards that measure and inform performance:
 \textbf{clinical dashboards}  provide clinicians with timely and relevant feedback on their patients' outcomes in order to inform decisions that improve the quality of patient care, while 
\textbf{quality dashboards} are meant to inform \textit{``on standardized performance metrics at a
unit or organizational level, to assist with operational decision making''}~\cite{dowding2015dashboards}. 
Successful examples of clinical dashboards include IDMVis~\cite{idmvis} and Composer~\cite{composer}. 
In IDMVis, Zhang et al. combined hierarchical task analysis~\cite{preece2015interaction} and abstraction~\cite{lam2018bridging} to understand hierarchies and sequences of tasks performed by clinicians working
with type 1 diabetic patients.
To develop Composer, Rogers et al. collaborated with medical experts to understand the tasks of orthopaedic surgeons working with a patient cohort who have undergone spinal procedures~\cite{composer}.



Unlike clinical dashboards, which cater to a specialized user group within specific clinical contexts, we focus on quality dashboards, which exhibit a much larger variety of users and contexts.
Originally derived from the concept of {\it balanced scorecards}~\cite{kaplan1992}, quality dashboards inherit several factors that are crucial to successful implementation and adoption.
These factors include scalability, flexibility of customisation, communication, data presentation, and a structural understanding of department-level and organization-level performance objectives and measures~\cite{assiri2006profit}. 
In our work, we show how to connect this structural understanding of these factors to visualization task classification, resulting in the development of a dashboard generation engine.
% the structural view of tasks, which has long been promoted by visualization task taxonomies and typologies~\cite{andrienko2006exploratory, meyer2015nested,brehmer2013multi, wehrend1990problem, amar1,kerracher2017constructing, ahn2014task,schulz2013design} and the advocacy for the benefits they present when used in early stages of visualization software design~\cite{sedig2013interaction, heer2012interactive, lammarsch2012developing, kerracher2017constructing}.



%\subsection{Visualization Authoring}



%We then sampled the task clusters to select a manageable number of representative tasks that could then be further discussed with stakeholders through two co-design workshops. 
%In the first workshop, we identified task compositions and sequences that constituted of a two-step hierarchy: a metric-level and an attribute-level. In the second workshop, we sought participant input to inform a mapping of this task hierarchy to a view specification hierarchy that can be reused to adapt different dashboards with varying metrics


%Figure~\ref{fig:flow} depicts the workflow of the TASHA framework. 
%Section~\ref{sec:dissect} describes the process of dissecting tasks, originally stated by users in natural language, in order to extract values for a task feature vector that would position each task in a 3D task space~\cite{BELIV}. 
%This positioning process enables us to identify clusters of tasks and to select a representative sub-sample of them which could then be presented to users at a co-design workshop for prioritization and task sequence generation. This latter process is described in Section~\ref{sec:codesign}.

%They argued that by setting out the range of potential tasks of interest (i.e. the task space), one may overcome known problems associated with simply asking people to introspect. Namely, the collected tasks may be incomplete due to the users' limited ability to introspect and articulate their needs, or they may be skewed towards a specific user group.
% Now to applications
%Existing research has consistently characterized different tasks' levels of \textit{abstraction} (e.g.~\cite{7061479, laha2015}) or \textit{granularity} (e.g.~\cite{brehmer2013multi,andrienko,book1} )
%A successful effort to bridge the gap between visualization and the domain of climate research was presented by Dasgupta et al.~\cite{7061479}.

%They have highlighted a number of threats to the validity of the task space created by qualitative methods alone such as interviews, observations, fly-on-the-wall and contextual inquiry. 
% 


%
% Amar and Stasko presented a taxonomy that focuses on users’ analytic primacy, which maps visualization tasks to  analytic goals, such as: exposing uncertainty, formulating cause and effect, and confirming hypotheses~\cite{amar3}.
 
%Through leading a cross-domain effort, they developed a classification scheme for visualization systems designed and developed by domain experts.
%Some of these feature vectors focused on the operational perspective, in which the focus is on \textit{how} tasks are performed~\cite{amar2}. 



==> tex/03_tschar.tex <==
%\textcolor{green}{READY FOR COMMENTS}

The input to the TASHA workflow is a corpus of qualitative user narratives that we collected through interviews and two National Clinical Audit datasets. This section describes these datasets and the process of characterizing the task space through mapping them to the AA task typology~\cite{andrienko2006exploratory}.
The outcome of this stage of the TASHA framework is a clustered view of the task space, which we used to reduce the number of tasks that in turn allowed us to facilitate further communication and co-design activities with project stakeholders (Figure~\ref{fig:flow}(a) and (b)). 


\subsection{TASHA Inputs: Datasets \& Interviews} 
\label{sub:data}

%The TASHA workflow is developed in the context of an interdisciplinary large-scale visualization project (QualDash) that aims to design, develop and evaluate a visualization dashboard tool to monitor healthcare performance metrics and improve the quality of care. 
 % from the School of Healthcare in our University.

\bstart{National Clinical Audit data}
Our team members from the healthcare sector supplied two datasets.
National Clinical Audits are databases commissioned and managed on
behalf of NHS England by the Healthcare Quality Improvement Partnership.
These databases are meant to systematically record and measure the quality delivered by clinical teams and healthcare organizations. 
Participating hospitals regularly contribute to updates of over 60 audits, with each audit focusing on a particular area of care or condition. 
We identified two audits of interest to the current phase of the project, with a vision for expansion to support more audits in the future. 
These two selected audits are the Paediatric Intensive Care Audit Network (PICANet) audit~\cite{picanet} and the Myocardial Ischaemia National Audit Project (MINAP) audit~\cite{minap}.
The choice of audits was made during the \textit{Cast} stage of Sedlmair et al.'s design study methodology~\cite{sedlmair2012design} and was based on data availability as well as access to data providers and stakeholders.
Due to the confidential nature of audit data, the audit providers provided us with simulated datasets representative of real audit data. 
%For PICANet, data is exported from individual PICU units across the country to the main audit database as XML files. Data exports must conform to the audit schema as defined in a centrally managed XML Schema Definition (XSD) document.
The PICANet schema definition contains a main \textit{``Admissions''} table that records 84 variables for each admission event. An additional 14 tables record information for referral and transfer events.   
In the MINAP audit, 140 variables are recorded for each admission event in a single spreadsheet. 
%The simulated data is based on real admissions and activity data between 2004 and 2014. No personal identifiers were retained in the simulation. % and a process of stratified randomisation for enumerated values and random addition/subtraction to continuous variables was carried out. %Extreme values were excluded. 
%Predicted probability of mortality was recalculated based on the randomly modified components of a risk adjustment model. 
%Only broad categories of diagnoses were retained. 
%MINAP suppliers provided a data definitions file, which we used to create a similarly simulated dataset. 
%This simulated dataset represents what is held by PICANet for this period but no single line of data could be back-traced to the original dataset.

\bstart{Interview corpus}
Our healthcare sector team members provided audio recordings and verbatim transcripts from 54 interviews with healthcare professionals spanning different backgrounds. Interview participants included 13 physicians,
15 nurses, 4 support staff,
2 board members,
8 Quality \& Safety staff,
6 Information staff and 6 participants with other diverse titles. 
The interview questions were designed to elicit the participants' own experiences with National Clinical Audit data, with an emphasis on the role of the data in informing quality improvement. 
Interviewees introspected and gave examples of when audit data was of particular use to them, where limitations and constraints arose, and what they would like to learn from the data in the future. 
% Interviews were audio recorded and transcribed verbatim. 

%The visualization team received interview data in the form of the raw transcriptions and a summary describing common themes. 
Given the transcriptions of these interviews, we asked: \textit{what is a minimalist set of tasks that should be supported by the dashboard in both audits? }
To answer this question, we tabulated all data-related use cases and questions from this transcript corpus.
We identified 127 unique questions about the data that were mentioned in interview transcriptions (78 tasks for PICANet and 49 for MINAP). 
We then sought to reduce this into a more manageable task space for the subsequent design phase of the project.
% This is where a typology-driven task characterization and clustering became crucial. 

\subsection{Characterizing the Task Space}
\label{sub:dissect}
% Why we chose this technique?
There were several common themes pertaining to information constructs among the 127 questions about data that we extracted from the interview corpus. However, when stated in natural language, the questions were phrased differently by different participants, which made it difficult to identify common patterns. 
We needed a way to map these statements to a structured task, which would allow us to cluster similar tasks. 
% We, therefore, positioned tasks collected in natural language along dimensions of the Andrienko and Andrienko task typology~\cite{andrienko2006exploratory} (hereafter referred to as the AA typology for brevity). 
The Andrienko and Andrienko task typology~\cite{andrienko2006exploratory} (hereafter referred to as the AA typology for brevity) satisfies this requirement as it proposes a structured mathematical formulation of tasks.
Andrienko and Andrienko also provide a relatively large list of natural text examples that we used to as a guide in our task analysis process. 
We recognize that their list is not exhaustive, as Lammarsch et al.~\cite{lammarsch2012developing} noted how their examples do not account for many tasks. 
However, this list provided a starting point to reason about tasks and their referential and characteristic components. %, and to understand what patterns may exist.
% It, therefore, facilitates our mapping from tasks expressed in natural language to vectors of tokens, which we used to group similar tasks. 

% We discussed the terminology  of the AA typology in Section~\ref{sub:aatt}.
In our notation inspired by the AA typology, we define four types of tokens that represent data components involved in {\it synoptic tasks}:

\begin{lstlisting}
<@\texttt{\textcolor{blue}{pattern\_k}}@> := <@$\mathbf{P(R_k)}$ @>
<@\texttt{\textcolor{blue}{reference(s)\_of\_set\_k}}@> :=  <@$\mathbf{R_k'} \mid \mathbf{R_k'} \subseteq \mathbf{R_k} $ @>
<@\texttt{\textcolor{blue}{characteristic\_i}}@> := <@ $c_i \in \mathbf{C}$ @>
<@\texttt{\textcolor{blue}{association\_j}}@> := <@ $ \beta(f(x) \mid x \in \mathbf{R_k'}) \approx \mathbf{P_{Assoc.}} $ @>

\end{lstlisting}

%\subsubsection{The AA Task Typology}
Where $\mathbf{P(R_k)}$ is a generic pattern (e.g., a trend) defined over the set of references $\mathbf{R}$ (e.g., months) of referrer type $\mathbf{k}$ (e.g., time).
The set $\mathbf{R_k'}$ is a subset of references in $\mathbf{R_k}$. For example, if $\mathbf{k}$ is time then $\mathbf{R_k'}$ can be a specific timestamp, a time range (e.g., a month or a quarter) or the entire period recorded in the data. 
To approximate natural language, we introduce the tokens \texttt{\textcolor{blue}{pattern\_k}} and \texttt{\textcolor{blue}{reference(s)\_of\_set\_k}} to represent  $\mathbf{P(R_k)}$ and $\mathbf{R_k'}$, respectively. 
Similarly, we use a token \texttt{\textcolor{blue}{characteristic\_i}} to represent
$c_i$, which is the $i^{th}$ characteristic in the set of all characteristics $\mathbf{C}$ in the data set. 

Lastly, we introduce the token \texttt{\textcolor{blue}{association\_j}} to represent a special type of pattern (an association) which can be used to constrain the elements of $\mathbf{R_k'}$.
In the AA typology, an \texttt{association} pattern regards a (sub)set of references as a
unified whole on the basis of similarity of their characteristics.
Formally, we define \texttt{\textcolor{blue}{association\_j}} as a pattern $\mathbf{P_{Assoc.}}$ which approximates a similarity behaviour that is defined over the subset $\mathbf{R_k'}$. 
%any constrained subset $\mathbf{R_k'}$ of the reference set $\mathbf{R_k}$ such that there exists a behaviour in the references in $\mathbf{R_k}$ that can be approximated with an association pattern $\mathbf{P_{Assoc.}}$. 
For example, the question \textit{``What is the proportion of children in the municipalities of Northern Portugal?''} %would be tokenized as \texttt{``What is the \textcolor{blue}{pattern\_1} of \textcolor{blue}{characteristic\_1} in \textcolor{blue}{association\_1} of \textcolor{blue}{reference(s)\_of\_set\_1}?''}; 
refers to an \texttt{\textcolor{blue}{association\_i}} pattern that constrains the subset of references (i.e., municipalities) considered to only those in Northern Portugal. 
Other types of patterns can be used as constraints. 
For example, we may consider \textit{``Northern Portugal''} to be an arrangement of locations. We may also think of it as a differentiation that separates the Northern municipalities from all others. 
To avoid overloading our notation, we use the token \texttt{\textcolor{blue}{association\_i}} wherever a pattern is used to \textit{reduce} the reference set $\mathbf{R_k}$ by constraining it to a range or to specific value(s). Any other occurrence of patterns in our tasks gets parsed as \texttt{\textcolor{blue}{pattern\_k}}.

 %The left hand side of these equations carries our introduced notation, which we describe as $tokens$ that represent typology components in the body of a task. The right hand side contains the mathematical notation used in the AA typology for the same components.
%Specifically, For example, ``discharge status'' is a characteristic of an admission event that records whether the patient was alive or not at time of discharge. 

%n addition to the $<\textcolor{blue}{pattern}>$ token, we further specify types of patterns wherever appropriate. For example, if a task specifies a pattern like ``months with high mortality'' or ``patients with a certain diagnosis'', we specify that the question expects an $<\textcolor{blue}{association\_pattern}>$ in this position. 
 
%Other pattern types include $differentiation$, $arrangement$ and $distribution$ $summary$~\cite{andrienko2006exploratory}. 


% \subsubsection{Mapping Tasks to the AA Typology}
% \label{sub:mapping}
%What have we done?

%To map tasks to their corresponding AA typology components, we first sought to extract tokens from the raw phrasing of each task. Given different styles of questions, we found that the same task can bear different interpretations and mappings. To reduce the uncertainty of the mapping, 
% To assess whether our introduced tokens can be used to extract the AA model components from natural text, 
% a sample list of questions was compiled by extracting the already-classified task examples from the Andrienko \& Andrienko book~\cite{andrienko2006exploratory}. 
Using our AA typology-inspired tokens, we parsed the 127 questions posed in natural language extracted from the interview corpus. 
We recorded the examples and their tokenized versions in a table, which allowed us to then arrange these tasks according to their similarity. 
\begin{table*}
	\caption{Examples of two task templates for \textsl{Behaviour Characterization} (BC) tasks, accompanied by analogous examples taken from the list provided by AA~\cite{andrienko2006exploratory} and tokenized versions two tasks (one for each audit). Square brackets delimit alternative tokens. Tasks related to the MINAP audit are labeled as TM\#, while tasks related to the PICANet audit are labeled as TP\#.}
	\label{tab:templates}
	\centering
	\scriptsize
	
	\begin{tabular}{|l|l|}
		\hline
		\rowcolor{light-gray} \multicolumn{2}{|l|}{
		\texttt{\textbf{BC1:} What is the \textcolor{blue}{pattern\_1} of [\textcolor{blue}{characteristic\_1}, \textcolor{blue}{association\_1}] of \textcolor{blue}{reference(s)\_of\_set\_1}   }}  \\   \rowcolor{light-gray} \multicolumn{2}{|l|}{\hspace{8mm}  
            \texttt{[over/per 
		\textcolor{blue}{association\_2} of \textcolor{blue}{reference(s)\_of\_set\_2}] ?}}
		\\
 \rowcolor{lighter} 
 \multicolumn{2}{|l|}{\textbf{Analogous AA example:} \textit{``What is the distribution of the population over the territory of Portugal?''}}  \\
 \hline
 \rowcolor{lighter} \textbf{\texttt{TM1:What is the number of inpatient mortality per month?}} & \textbf{\texttt{TP1:What is the raw death count in patients per month?}} \\
         \hspace{4mm} \texttt{\textcolor{blue}{pattern\_1} := count} & 
         \hspace{4mm}
         \texttt{\textcolor{blue}{pattern\_1}} := count \\
         \hspace{4mm}
          \texttt{\textcolor{blue}{association\_1} := deceased} &  \hspace{4mm} \texttt{\textcolor{blue}{association\_1} := deceased} \\
          \hspace{4mm}
          \texttt{\textcolor{blue}{reference(s)\_of\_set\_1} := patient admissions} & \hspace{4mm} \texttt{\textcolor{blue}{reference(s)\_of\_set\_1} := patient admissions}\\
          \hspace{4mm}
          \texttt{\textcolor{blue}{association\_2} := months} & \hspace{4mm} \texttt{\textcolor{blue}{association\_2} := months}\\
          \hspace{4mm}
          \texttt{\textcolor{blue}{reference(s)\_of\_set\_2} := time of admission} &  \hspace{4mm} \texttt{\textcolor{blue}{reference(s)\_of\_set\_2} := time of admission} 
         \\ 
		 \hline
         \multicolumn{2}{l}{} 
         \\ \hline
		 \rowcolor{light-gray} \multicolumn{2}{|l|}{\texttt{\textbf{BC2:} On a given \textcolor{blue}{pattern\_1} of [\textcolor{blue}{association\_1}, \textcolor{blue}{characteristic\_1}] in \textcolor{blue}{reference(s)\_of\_set\_1},  }} \\   \rowcolor{light-gray} \multicolumn{2}{|l|}{\hspace{7mm} 
		  \texttt{ what is the \textcolor{blue}{pattern\_2} of [\textcolor{blue}{characteristic\_1} or \textcolor{blue}{characteristic\_2}] [over \textcolor{blue}{association\_2}\textcolor{blue}{reference(s)\_of\_set\_2}]?} }
		 \\
	    \rowcolor{lighter} 
	    \multicolumn{2}{|l|}{
	    \textbf{Analogous AA example:}  \textit{``In districts with high proportions of children in Northern Portugal, what is the average proportion of children?''}} \\ 
	    \hline
		\textbf{\texttt{TM2: On a month with high mortality rate, }} & \textbf{\texttt{TP2: On a month with high mortality rate,}} \\
		\textbf{\texttt{what is the average length of stay?}} &  \textbf{\texttt{what is the case mix?}}  \\
		\hspace{4mm}
		\texttt{\textcolor{blue}{pattern\_1} :=  count}  & \hspace{4mm}
		\texttt{\textcolor{blue}{pattern\_1} :=  count} \\
        \hspace{4mm}\texttt{\textcolor{blue}{association\_1} := deceased}  & 
        \hspace{4mm}\texttt{\textcolor{blue}{association\_1} := deceased}
        \\ 
        \hspace{4mm}
        \texttt{\textcolor{blue}{reference(s)\_of\_set\_1} := patient admissions} &
        \hspace{4mm}
        \texttt{\textcolor{blue}{reference(s)\_of\_set\_1} := patient admissions}
        \\ 
        \hspace{4mm}
        \texttt{\textcolor{blue}{pattern\_2} = average} &
        \hspace{4mm}
        \texttt{\textcolor{blue}{pattern\_2} = distribution}
        \\ 
        \hspace{4mm}
        \texttt{\textcolor{blue}{characteristic\_2} :=  length of stay} & \hspace{4mm}
        \texttt{\textcolor{blue}{characteristic\_2} :=  primary diagnosis} \\
        \hspace{4mm}
        \texttt{\textcolor{blue}{association\_2} := months} & \hspace{4mm} \texttt{\textcolor{blue}{association\_2} := months}
        \\
        \hspace{4mm}
         \texttt{\textcolor{blue}{reference(s)\_in\_set\_2} := time of admission} & \hspace{4mm}
         \texttt{\textcolor{blue}{reference(s)\_in\_set\_2} := time of admission} \\


		
		\hline
	\end{tabular}
	\vspace{-5mm}
\end{table*}

Table~\ref{tab:templates} shows two example task templates. Each is accompanied by an analogous AA example and two tokenized tasks, one for each audit. For an expanded listing of templates and examples from the AA model and from our tokenized tasks, refer to our Appendix A in supplementary material. 
The task templates $\mathbf{BC1}$ and $\mathbf{BC2}$ in Table~\ref{tab:templates} are both {\it Behaviour Characterization} tasks, in which reference subsets are the input and a particular pattern is the output. 
The $\mathbf{BC1}$ template can be illustrated with the AA example:
\textit{``What is the distribution of the population over the territory of Portugal?''}.
This example inquires about a pattern (distribution) of a characteristic (population size) over a reference set (territory of Portugal). 
The $\mathbf{BC1}$ template shows additional optional tokens in square brackets. This indicates that the question may include more than one reference set, as in the example \textit{``How does the distribution of the population over the territory of Portugal vary over time?''} in which months or years can be associations of references in the set \texttt{time}. Other optional tokens include associations that can constrain some of the task's reference sets. For example, the task may inquire about the distribution within specific municipalities of Portugal over a specific period of time. 

When applied to our coded interview corpus, the template $\mathbf{BC1}$ makes it straightforward to extract tokens from a naturally expressed task. Tasks $\mathbf{TM1}$ and $\mathbf{TP1}$ in Table~\ref{tab:templates} are examples of questions that interviewees asked in regards to the two audits. In both tasks, an association is used to reduce the reference set containing all admitted patients to only the deceased ones. The question then inquires about a distribution summary pattern (count) aggregated over the admissions (reference set 1) in monthly associations of time (reference set 2). 

 
Similarly, the template $\mathbf{BC2}$ can be likened to another AA example: 
\textit{``In districts with high proportions of children in Northern Portugal, what is the average proportion of children?''}. 
Here the $districts$ form a set of references, which are associated by the constraint $North$ $of$ $Portugal$.
Initially, the question specifies a pattern defined by $high$ values in the characteristic $child$ $proportion$  over the reference subset resulting from the association constraint (i.e., districts in Northern Portugal).
The question then refers to a distribution summary pattern (\texttt{average}) of the same characteristic. %Note that in this case, the question uses the same characteristic in both parts of the question. 
% In some AA examples, the question sometimes introduces a new characteristic (e.g., \textit{``the proportion of elderly people''}). 
% The additional square brackets at the end of the template are meant to cover these other possibilities. 

Applying the template to $\mathbf{TM2}$ and $\mathbf{TP2}$ from our interview data (see Table~\ref{tab:templates}), we can understand that the task requires us to look at the references in the set of \texttt{patient admissions} associated by the fact that the patients are \texttt{deceased}. Initially, the question specifies a pattern of high \texttt{count} on the reference subset resulting from the association. The question then  inquires about a distribution summary pattern (an \texttt{average} in $\mathbf{TM2}$ and a \texttt{distribution} in $\mathbf{TP2}$) defined over some characteristic within monthly associations of time.  

%Both examples are classified as synoptic Behaviour Characterization (BC) tasks,
% why are they synoptic tasks?
%These tasks are synoptic, meaning that they consider sets of references as a whole. 

%In our case, data is stored as individual admission events. Therefore, tasks considering monthly aggregates or patients in a specific category (e.g. deceased) as a unit of information are classified as synoptic rather than elementary tasks.  
%We use numbers at the end of each token because tasks are expected to include multiple different occurrences of a token type. For example, tasks $T1$ and $T2$ above both include two referrer types (time and admission events). The numbers in $<\textcolor{blue}{reference(s)\_of\_set\_1}>$ and $<\textcolor{blue}{reference(s)\_of\_set\_2}>$ reflects this difference. We apply the same logic for characteristics. 

%We note here that if the data was stored as monthly aggregates, it would have been possible to consider these as elementary tasks. However, because the data is stored on a per admission event basis, subsets of data records (i.e. monthly aggregates) need to be taken and regarded as a whole when answering these questions. Hence, we classify them under the synoptic category. 


%
% Explain template notation (tokens) here
%As mentioned earlier, these templates are derived from the wording of task examples in the AA book. The first template is derived from the task 
%TODO: cite the book pages here

The purpose of our task templates is structure rather than coverage. 
Rather than proposing a new task space, we adopt the structure of the AA typology %Actual phrasing of the tasks may slightly vary. For example, the example starting with \textit{``In the cluster with...''} is mapped to a template that starts as \textit{``On a given $<\textcolor{blue}{association\_pattern}>$...''}. This is to clarify to the analyst that tasks in this category expect an association pattern as input.
%Let us now define what each token means. The token $<pattern>$ is a generic one describing any type of pattern that characterizes behaviour in the data.
%Different types of patterns include $association$, $differentiation$, $arrangement$ and $distribution$ $summary$.  
%A $differentiation$ pattern describes the variation of references based on differences in their characteristics. 
%An $arrangement$ considers order (e.g. a trend), and a $distribution$ $summary$ contains descriptive statistics (e.g. sum, count, average, etc.).
%In our template definitions, we use the token $<\textcolor{blue}{pattern}>$ where any type of pattern can be inserted in the task structure. 
%Where the template assumes a specific pattern type, we include the type in the token (e.g. $<\textcolor{blue}{association\_pattern}>$). 
%Other tokens include characteristics and references extracted from reference sets. 
%Table S1 (see Supplumental Material) contains the full list of synoptic task templates, along with examples (from the book), and MINAP-related tasks (from interviews) in each category. It further lists the different data model components extracted from each task, based on this dissection. 
% How can this help? 
% Task composition
%By regarding tasks in the context of their corresponding templates in this manner, the process of extracting referrers, characteristics, and relation components was greatly simplified. 
to identify recurring patterns. For example, in Table~\ref{tab:templates}, we show that the reference sets \texttt{patient admissions} and \texttt{months} and the association \texttt{deceased} are repeated in all tasks.
This is an indication of a possible connecting structure between tasks. 
$\mathbf{TM1}$ can be seen as a sub-task of $\mathbf{TM2}$: one needs to be able to understand the patterns of monthly death count in order to identify a month with high mortality. The same connection is apparent between $\mathbf{TP1}$ and $\mathbf{TP2}$.

%Another advantage of this typology-driven approach is that grouping tasks by their corresponding templates provided a finer grained classification within each category, so tasks of similar structure were placed in close proximity to each other. 
%This understanding guided our design choices. For example tasks like $T12 - T15$ in Table S1 
 %are grouped together. Each one of these tasks can be addressed with a visualization that displays monthly aggregates of a single variable, implying similar design choices for each. 

% What are the outcomes?


\bpstart{Task space clusters}
\label{sub:clusters}
Our task characterization process eventually revealed the overall structure of our task space. 
By placing the task feature vectors along rows of a table, we could readily identify similarities and differences across tasks. 
To do so, we replaced the names of individual referrers and characteristics with their respective data types. 
Of the 78 tokenized tasks produced for PICANet, 31 involved observing a quantitative variable over time, 17 involved observing a quantitative variable grouped by a nominal one, and 18 involved comparing up to three quantitative variables in conjunction.
Of the 49 tokenized tasks produced for MINAP, 10 involved monitoring a quantity over time, 21 involved monitoring a quantity grouped by a nominal variable over time, and 3 involved identifying relations between up to two quantities. 
%98\% of the tasks dealt with aggregate-level data (no patient-level data was required) at a monthly scale. 
This data abstraction allowed us to place tasks along the $Type$ $Cardinality$ dimension of Elshehaly et al.'s three-dimensional task space~\cite{elshehaly2018taxonomy}, which groups tasks having similar numbers and types of variables.
Finally, we excluded 11 PICANet-related tasks and 15 MINAP-related tasks, because they inquired about variables that were not captured in the audits, such as details about clinicians or the number of beds.

Given our structured representation of tasks along with our data abstraction, we concluded that the interviewees were primarily interested in temporally aggregated (synoptic) patterns in the data.
Specifically, 95\% of PICANet tasks and 89\% of MINAP tasks inquired about monthly aggregates over a year span. About 5\% of the tasks in both audits involved comparing against historic data spanning 3 to 5 years at different levels of temporal granularity.    
By grouping tasks with similar data abstractions, we were able to reduce the task space and select representative tasks that could then be in further discussions with stakeholders. 

 %are seeking to understand the values of the output characteristic. They may wish to monitor the change in these values over time or their distribution across different groupings. Mapping this type of tasks to the corresponding feature vector is as simple as identifying the $<reference(s)>X$ and $<characteristic(s)>$ components and specifying the data types, granularity and targets for these components. 

%Notice that the type cardinality of a task can be inferred from the specification given so far. For example, through looking at the the aggregates vector, one can see that the first variable is a temporal one and that the other two variables are quantitative. 


%We begin by mapping an input task to the most similar task template in the table. This matching is currently done manually, but could potentially be aided with NLP techniques. TODO: like what?





% Output: a structured view of the task space that enables task clustering and sampling
% (1) Identified task clusters
% (2) Identified goals: - Assess performance indicators (metrics) - Assess data quality - Root cause analysis

%\subsubsection{Further Task Classification}


==> tex/04_sampling.tex <==
%\textcolor{green}{READY FOR COMMENTS}

\begin{figure*}[b!]
 \vspace{-5mm}
 \centering 
    \subfloat[\label{left}]{
        \includegraphics[width=.32\linewidth, height=1.6in]{pictures/ctb1-1.jpg}
    }
    \hfill
    \subfloat[\label{center}]{
        \includegraphics[width=.32\linewidth, height=1.6in]{pictures/CTB1_-1.jpg}
    }
    \hfill
    \subfloat[\label{right}]{
        \includegraphics[width=.31\linewidth, height=1.6in]{pictures/ctb2-1.jpg}
    }
 \caption{Example participants' responses from: (a) and (b) Session 1 -- Task Contexts; and (c) Session 2 -- Task Sequences.} 
 %TODO: Scan these for better image quality
 \label{fig:activ1}
\end{figure*}

Our structured analysis of tasks based on the AA Typology revealed commonalities across the many tasks collected from interview participants. 
The next step was to use these commonalities to sub-sample the task space by selecting representative tasks from each group of task clusters. 
This process was easier for the task templates associated with a small number of instance tasks.  
However, templates such as $\mathbf{BC1}$  (in Table~\ref{tab:templates}) was associated with 
%26 instances in MINAP and 31 instances in PICANet
more than twenty tasks in each audit, and thus we carefully considered how to avoid missing important tasks.
% and potentially distinct task. 
We therefore subdivided task groups that contained a large number of tasks. 
This subdivision was based on the type of main output pattern in {\it Behaviour Characterization} and {\it Direct Comparison} tasks, or based on the type of input in {\it Pattern Search}, {\it Inverse Comparison} or {\it Relation Seeking} tasks.
Rather than regarding patterns at a high level of abstraction (e.g., association, differentiation), we looked at the specific patterns mentioned in relation to distributions, proportions, percentages, trends, and the like. 
%After this latter subdivision, the number of tasks falling within each group reduced to less than 5 in each category. 
%To further reduce heterogeneity in the resulting clusters, we further considered the $Type$ $Cardinality$ dimension of Elshehaly et al.'s three-dimensional task space~\cite{elshehaly2018taxonomy}, which groups together tasks having similar numbers and types of variables. 

At the end of the task clustering process, tasks within each cluster exhibited a high similarity in their structure and in terms of the variables involved. %However, they varied in the choice of variables involved (referrers and characteristics). 
We prioritized tasks within each cluster and selected up to five representative tasks from each. %template group. 
This prioritization was facilitated by the fact that tasks were represented by their feature vectors of token values (as shown in Table~\ref{tab:templates}). For clusters containing three or more tasks, we considered the names of their referrer(s) and characteristic(s). We then performed a word search of these names in the interview transcripts, and names that were mentioned more frequently were used to prioritize tasks within a cluster. 
As a result of this process, we were able to reduce the size of the task space to 23 tasks for both audits (from the original set of 127 tokenized tasks). 
% This reduced task set was then fed into the next stage of the TASHA workflow, which aimed to put these tasks together in context and understand connections and sequences among them. 
%validate the priorities of the set of tasks that will be taken forward to the design stage of the dashboard, and explore sequences among them. 

==> tex/05_codesign.tex <==
%TODO: Explain that we had to strip the tasks out of their context and use the decomposition of task outcomes (more than one unknown were split) 

% \begin{figure*}[b!]
%  \vspace{-5mm}
%  \centering 
%     \subfloat[\label{left}]{
%         \includegraphics[width=.32\linewidth, height=1.6in]{pictures/ctb1.pdf}
%     }
%     \hfill
%     \subfloat[\label{center}]{
%         \includegraphics[width=.32\linewidth, height=1.6in]{pictures/CTB1_.pdf}
%     }
%     \hfill
%     \subfloat[\label{right}]{
%         \includegraphics[width=.31\linewidth, height=1.6in]{pictures/ctb2.pdf}
%     }
%  \caption{Task Contextualization Examples (Activity 1).} 
%  %TODO: Scan these for better image quality
%  \label{fig:activ1}
% \end{figure*}

%\textcolor{red}{UNDERGOING REVISION}

%input at this point
% The sub-sampled task space obtained via the process described in Section~\ref{sec:sampling}
% contains a list of 23 representative tasks. %each featuring
%\begin{itemize}[noitemsep,nolistsep,leftmargin=*]
   % a unique task template. %, and a feature vector containing the task's tokens and their assigned values and data types. 
%\end{itemize}
%We further regard the task structures in light of the data types involved in their referrer and characteristic tokens. 
%This list presents a manageable subset of tasks which can be taken forward to specify visualization and functionalities required in the dashboard. 
Each of our 23 representative tasks can be answered individually with a visualization displaying up to three metrics over time.
% (maximum feature vector length). % and that a vast majority of tasks involve monthly aggregates (i.e. with association\_i = month). 
For any of these tasks, one could, in theory, produce an independent visualization along with functionality to modify the displayed metrics. %to support other tasks, which were not included in the reduced task space. 
For example, the task \texttt{TM1} in Table~\ref{tab:templates} can be addressed with a simple bar chart showing monthly mortality counts. Additional functionality can modify the \texttt{mortality} metric to other quantitative metrics (e.g., \textit{service delays}) that correspond with the same task template (i.e., \texttt{"What is the count of delayed patients per month?"}). 

However, interviewees posed multiple questions and were interested in multiple metrics, which limits the effectiveness of independent visualizations.
%Given the relatively small number of referrers and characteristics in our task Each unique task structure can be supported with a single visualization view displaying the metrics listed in the task's feature vector, along with functionality to change the metrics displayed to any of the other metrics mentioned in the task's corresponding cluster. 
%For example, the tasks $T12 - T15$ in Table S1 can use a simple bar chart showing the corresponding measure. In a requirements specification, we could potentially specify that the initial view of the dashboard must display the metric that is most inquired about (e.g. mortality in this case) and add a selection menu for users to switch to any of the other mentioned measures. However, this solution 
Dashboards enable people to see multiple metrics together, compare them with one another, and answer a sequence of related questions, toward an understanding of the so-called {\it big picture}. 
Within a dashboard, we must pay special attention to the \textit{groupings} and \textit{sequences} in which tasks are performed.
A \textit{grouping} of related tasks may imply juxtaposed visualizations, while a \textit{sequencing} relationship implies view transitions or transformations. 
The tokenized task space we defined in the previous section revealed potential task groupings and sequences based sets of common data metrics (e.g., tasks \texttt{TM1} and \texttt{TM2} in Table~\ref{tab:templates}). 

\subsection{Co-Design Workshop}
\label{sub:material}

There is a danger in relying on our data-centric view of tasks, as it can lead to design decisions that do not match users' analysis processes.
To better understand the connection between tasks, we conducted a full-day co-design workshop to elicit task groups and sequences.  
%Connections like the ones made between $T1$ and $T2$ in Section~\ref{sec:tschar} are possible to be made in the complete task space but are not necessarily visible in the sub-sampled space, because the choice of metrics used in the representative subset may not be consistent across clusters. 
%In order to reason about the sequences and connections among tasks, 
%We organised a two-session co-design workshop to conduct these activities. 
Workshop participants were seven healthcare professionals having both clinical and non-clinical backgrounds (3 hospital information managers, 2 consultants and 2 nurses). 
%We elicited two levels of task prioritization through the two sessions of the workshop, with the anticipation that understanding tasks in a two-step sequence can inform a high-level design perspective on
%The first activity of the workshop aimed to elicit context of use around each of the tasks in the reduced task space and understand their connection, with the anticipation that understanding these connections will inform view layout on the dashboard.
%The second activity aimed at eliciting task sequences, in order to determine 
%whether the dashboard should be of the \textit{visual} or the \textit{functional} genre, as defined by Sarikaya et al.~\cite{sarikaya2019we}.
%We anticipated that the former would be appropriate if task sequences can fit on one screen, while the latter would be the correct choice if the sequences require interaction to support multi-step viewing, and possibly different levels of detail. 
%To run these activities, two workshop sessions were organized, as will be described shortly. 

To elicit stories about tasks, we designed and printed ``task cards''. Figure~\ref{fig:activ1} shows two example task cards ((a) and (b)) along with participants' responses. 
Each task card contains only one task and is subdivided into four main sections used to collect contextual information about the task.
The header of a card contains the task's body and an empty box for participants to assign a relevance score. Three parts of the card are dedicated to elicit information about the ways in which this type of question is answered in current practice: the time it takes, the data components used, and any textual information that might be involved.
The majority of space on the card is dedicated to the fourth section labeled as ``sketches''. This section of the card provides a space for participants to sketch out the processes involved in answering the question, and visualizations (if any) that are used in the same context. 
% Each task card was printed on a separate A3 paper.  

We divided participants into two groups and assigned each a task subset from one of the audits. 
We assigned participants to groups such that each group included people who are acquainted with the audit. 
Two project team members facilitated the discussion with each group over the course of two sessions.  

\label{sub:proc}
\bpstart{Session 1\,---\,Task Contexts}
We first presented all task cards for the audit and asked participants to perform a sequence of steps
%\begin{enumerate}[noitemsep,nolistsep,leftmargin=*]
beginning with selecting relevant task cards that resonated with them given their current practice. In addition to the card stack on each table, we gave each participant two blank cards that were partitioned in the same manner but contained no text in the question field. Participants could either select a relevant task from the stack or write their own on a blank card. 
They were also asked to rephrase any question posed on a card. 
We further asked that participants select as many cards as they felt were relevant while prioritizing the most important ones.
We asked them to fill out their selected card(s) individually at first and then add more information during a group discussion.
We then asked them to place the card(s) on one of the four corners of the table. Each corner was labelled with one of four user groups that we identified in the interviews corpus: clinical teams, clinical service units, quality and safety committees, and a trust board. Finally, we asked participants to place a card closest to the user group that they felt the task was most relevant to. 
%\end{enumerate}

%Similar to a user-story generation workshop~\cite{cohn2004user} and 
Inspired by Brehmer and Munzner's approach to task analysis~\cite{brehmer2013multi}, we asked participants to answer three questions:
\textit{why} these tasks are important, 
\textit{how} these tasks are currently performed, and
\textit{what} information needs to be available to perform the task (\textit{input}) as well as \textit{what} resulting questions might arise after completing the task (\textit{output)}.
Additionally, to support context generation, we added a \textit{who} dimension inspired by agile user story-generation workshops~\cite{cohn2004user}.
 
 \bpstart{Session 2\,---\,Task Sequences}
The second session aimed to obtain \textit{entry-point} tasks, tasks that initiate a task sequence that can be accomplished at a glance without directly interacting with a dashboard interface. 
To identify these tasks, we returned the prioritized task cards from Session 1 to participants along with a consolidated index of selected tasks. 
%The steps that participants were requested to follow for this activity were to: 
We asked participants to perform the following: 
\begin{enumerate}[noitemsep,nolistsep,leftmargin=*]
    \item \textit{From the list of prioritized tasks, select the most pressing questions to be answered at a glance in a dashboard;}
    \item \textit{Merge tasks that are likely to be answered together;} 
    \item \textit{Sketch the layout of a dashboard that could provide the minimally sufficient information for answering these tasks.}
\end{enumerate}
While this co-design workshop elicited interface sketches from participants, the primary purpose of this session was not to collect design alternatives but rather to seek an understanding of task sequences and relationships from participants' perspectives.

\begin{table*}[b!]
% 	\vspace{-5mm}
	\caption{A list of tasks relating to the \textsl{Call-to-Balloon} metric.}
	\label{tab:mort}
	\centering
	\scriptsize
	\resizebox{0.9\textwidth}{!}{%
	\begin{tabular}{|c|l|c|c|c|c|}
		\hline
		 \textbf{Code} & \textbf{Task} & Q & N & O & T \\
		\hline
		\hline
		\texttt{TM3:} & \textbf{Entry-point:} \textit{What is the number of delays and PCI patients per month?} & 2 & & & 1 \\
		\hline
		& \textbf{Subsidiaries:} &  & & &  \\
		\texttt{TM3.1}&	\multicolumn{1}{|l|}{\textbullet~\textit{On a given month, what is the percentage of patients meeting target Call-to-Balloon time?} } & + 1  &  & &  \\
	    \texttt{TM3.2} & \multicolumn{1}{|l|}{\textbullet~\textit{Of patients that did not meet the Call-to-Balloon target, which ones were direct/indirect admissions?}  } &  & + 1 & &  \\
		\texttt{TM3.3} & \multicolumn{1}{|l|}{\textbullet~\textit{Of patients that did not meet the target, which ones commuted from a far away district?}  } &  & + 1 & &  \\
		\texttt{TM3.4} & \multicolumn{1}{|l|}{\textbullet~\textit{ For a month with a high number of delays, what was the average door-to-balloon time?}  } & + 1  & & &  \\
		\texttt{TM3.5} & \multicolumn{1}{|l|}{\textbullet~\textit{How does a month with high number of PCI patients compare to the same month last year?} } &  &  & & +1  \\
	    %$TM5$ & \multicolumn{1}{|l|}{\textbullet Are the majority of patients leaving the hospital alive or dead? [SBC6] } & + 1  &  & & \\
		\hline
	\end{tabular}
	}
\end{table*}

\subsection{Co-Design Workshop Results}
\label{sub:wres}
%\textcolor{red}{NEW Section content}

\bstart{Task contexts}
% What we learned
Our analysis of sketches, our notes and the workshop participants' comments revealed three main ways to characterize groups and sequences of tasks:
\textbf{Finding 1:} Individual metrics have independent task sequences.
\textbf{Finding 2:}  Each metric has an entry-point task that combines a number of measures (i.e. variables) to be monitored over time. 
% sometimes compared to a national target.
\textbf{Finding 3:} After the entry-point task, investigation of further details involves one or more of three {\it subsidiary Tasks}: 

\begin{itemize}[noitemsep,nolistsep,leftmargin=*]
    \item \texttt{ST2}: \texttt{Compare with metric-related \textbf{measures} }
    \item \texttt{ST1}: \texttt{Break down into \textbf{categories} }
    \item \texttt{ST3}: \texttt{Expand to different \textbf{time units} }
\end{itemize}

For example, we highlight the \textit{Call-to-Balloon} metric from the MINAP audit. 
The \textit{Call-to-Balloon} metric measures the interval between the call for help (i.e., an ambulance) and the start of Primary Percutaneous Coronary Intervention (PCI), a balloon that is used to relieve the narrowing in an artery.
For this metric, participants in the MINAP group explained that they look at monthly counts and percentages of delayed cases, along with the total number of admitted PCI patients. % (i.e. ones that did not meet a nationally defined target of 150 minutes).
They then link this knowledge to a breakdown of known delay causes to decide whether or not they were justified. 
The participant response shown in Figure~\ref{fig:activ1}(a) depicts this contextual linkage. 
In Figure~\ref{fig:activ1}(b), another participant linked the same metric to historic information investigating data from previous years. 
These and similar links were constructed by participants in the first session of the workshop, which revealed a lack of overlap across the metrics. For example, no mortality information was discussed in the context of delays (\textbf{Finding 1}).
% The supplementary material provides a similar analysis of other metrics.

When asked in the second session to combine tasks from all metrics into an initial dashboard view, this lack of overlap persisted in many of the designs. Participants typically chose one metric and faceted views of different measures pertaining to the metric. An example is shown in Figure~\ref{fig:activ1}(c), in which a participant drew a layout consisting of five views relating to the \textit{Call-to-Balloon} metric and an information box (bottom right) that shows data quality information. 
In another sketch, a participant focused exclusively on data quality and sketched different views pertaining exclusively to it. 
Of the participants who sketched multiple metrics, one used a minimalist representation (buttons with metric names on each) to be shown on a dashboard's home screen, stating that \textit{``I want something very simple that will tell me where something is wrong in a metric, then I can click and find out more''}. 

Within each metric, we also found a great amount of consistency in the way that participants sketched task sequences. An entry-point task  for the \textit{Call-to-Balloon} metric combined two tasks matching the \texttt{BC1} template from Table~\ref{tab:templates} (\textbf{Finding 2}).
This is reflected in the
monthly bar charts showing aggregates of patient counts who did and did not experience delays (See Figure\ref{fig:activ1}(a) and (b)). After this entry point task, different areas of concern arise. We summarize these subsidiary tasks and their data types in Table~\ref{tab:mort} (\textbf{Finding 3}).



%These contexts offered links between the tasks in our task space and enabled us to extract groups of referrers and characteristics that can be shown together on the dashboard, as will be discussed in Section~\ref{sec:metric}. 

Participants identified 5 metric entry point tasks for the MINAP audit and 6 for PICANet audit. 
Despite the variability of individual metrics for each audit, the structure of entry point tasks remained constant across metrics and across audits.
Namely, they combined one or more associations of references to monitor their patterns over time (task template \texttt{\textbf{BC1}}). 
We refer to tasks that follow entry-point tasks as {\it subsidiary tasks}, which rely upon the identification of a reference subset (e.g., admissions in a month) or a characteristic pattern (e.g., high mortality) in the entry-point task. 
Subsidiary tasks add measures to investigate related areas of concern or interest.
To demonstrate this relationship, we show the \textit{Call-to-Balloon} entry-point and subsidiary tasks in Table~\ref{tab:mort}.
%, and a full list of all metrics and their corresponding hierarchies can be found in Table S2 (see Supplemental Material). 
We also augment this entry-point to subsidiary task sequence with additional information that we use to guide our dashboard design decisions. %Namely, each task is followed by the template code which positions it in the AA Typology. This information can help us understand which of these tasks are comparison tasks ([SCOM]),  Behaviour Characterizations tasks ([SCB1], [SBC5] and [SBC6]) and which are Relation Seeking tasks ([SRS]).
%This understanding can further help us understand the types of patterns involved (e.g. trends, distributions, summaries, etc.). 
%Namely, we explored the position of these tasks along the type cardinality dimension the the $3D$ task space in~\cite{elshehaly2018taxonomy}. 
The four rightmost columns in Table~\ref{tab:mort}
show how many Quantitative (Q), Nominal (N), Ordinal (O) and Temporal (T) variables are involved in each task. 
For the \textit{Call-to-Balloon} metric, the entry-point task involves identifying how two quantities trend over time: the count of delays and the count of PCIs. 
The subsidiary tasks typically involves adding one or two more measures. 
%For example, to understand patterns in length of stay, in the context of deceased patients or of a months with high mortality, one first needs to detect an association between references (admissions) where patients were deceased and/or between months which had large numbers in this association pattern.  
%Next, one needs to add the quantitative measure (length of stay) to the context defined by this association to understand what patterns may arise. 
%Similarly some tasks require the addition of nominal or temporal variables. For example, the last two tasks require the addition of further temporal granularities (e.g. years and quarters). 

We emphasize that some dashboards may involve a larger number of measures or data dimensions than what we consider here. However, our analysis in the context of healthcare quality monitoring reveals that tasks rarely ever involve more than four measures. %We note here that by variables we mean referrers and characteristics that are displayed in the visualization. Some of these variables may be computationally derived from multiple database attributes. If there is no need to visualize the original attributes from which the variable was derived, we do not count them in our type cardinality classification of a task. 

%In addition to the structural benefits of this typology-driven approach to task analysis,task hierarchies have revealed such findings as the fact in a typical usage scenario, audits rarely interact and metrics within an audit have limited interactions among themselves. This is especially true from a clinical governance perspective (for clinical teams and clinical service units). 
%In these usage scenarios, users are interested in an initial high-level view of all metrics for monitoring purposes. Once an area of concern is identified, users would like to examine metrics individually, separate from other metrics on the dashboard. 

%\bstart{Assessing task space coverage}Out of 23 tasks that were presented to participants, 17 tasks were selected and prioritized from this set (true positive). Additionally, participants added 6 more tasks that were not captured in the sub-sampled task space (false negative).This means that our task space sub-sample captured the tasks of interest to workshop participants at around 74\% sensitivity. 

==> tex/061_mss.tex <==
%%%%%%%%% Moved from intro.tex 
% TODO: rearrange text here to see where this goes

We define the Metric Specification Structure (MSS) shown in Figure~\ref{fig:flow}(e) as a JSON structure that aims to configure the visualizations shown in a single expandable metric card.
To configure an entire dashboard, we feed an array of MSSs to our visualization engine, which creates a metric card for each MSS in the array. 
Each metric card expands into four views (Figure~\ref{fig:ctb}) that are configured by the corresponding MSS. 
% An MSS formalizes the entry-subsidiary task structure identified for each individual metric into a format that can be ingested by  visualization engine.
The use of JSON to customize visualization views is inspired by Satyanarayan et al.'s Vega-Lite grammar ~\cite{vega}.  
Vega-Lite is intended for general-purpose design of interactive statistical charts, providing considerable visual expressivity.
For dashboard generation, we consider a constrained design space relative to Vega-Lite that: \textit{(a)} simplifies view specification for entry-point tasks, and \textit{(b)} expands the functionality of Vega-Lite's view concatenation to support views of subsidiary tasks related to each metric. 
 
%To generate a dashboard, we feed an array of MSSs to the dashboard generation engine, described in Section~\ref{sub:generate}, which in turn generates the corresponding metric cards on the dashboard. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{table*}[b!]
	\caption{Mapping the entry-point task in Table~\ref{tab:mort} and its subsidiary components to the corresponding Metric Specification Structure.}
	\label{tab:mss}
	\centering
	\scriptsize
	
	\begin{tabular}{|ll|}
		\hline
		\rowcolor{light-gray} \multicolumn{2}{|l|}{
		\texttt{\textbf{Task:} What is the number of delays and PCI admissions per month? }}  \\ 
		\hline
 \rowcolor{lighter} AA Model Tokens & Metric Specification Structure(MSS)   \\
 \hline
         \hspace{4mm}\texttt{\textcolor{blue}{reference(s)\_of\_set\_2} := time of admission} & \textcolor{gray}{1.} \hspace{4mm} \texttt{\{"\textcolor{blue}{x}" : "date/time arrival at hospital",} \\
         \hspace{4mm}
          \texttt{\textcolor{blue}{association\_2} := months} & \textcolor{gray}{2.} \hspace{6mm} \texttt{"\textcolor{blue}{timeUnit}" : "month",}\\
          &\textcolor{gray}{3.  }\hspace{6mm}\texttt{"\textcolor{blue}{xtype}" : "temporal",}\\
          & \textcolor{gray}{4.} \hspace{6mm}\texttt{"\textcolor{blue}{xlabel}" : "year",}\\
          \hline
         \hspace{4mm}
          \texttt{\textcolor{blue}{reference(s)\_of\_set\_1} := patient admissions}
          & \textcolor{gray}{5.}
          \hspace{6mm} \texttt{"\textcolor{blue}{y}" : ["ctb", "pci"],}\\
         \hspace{4mm}
          \texttt{\textcolor{blue}{association\_1\_1} := delay > 150} 
          & \textcolor{gray}{6.} \hspace{6mm} \texttt{"\textcolor{blue}{yfilters}" :[\{"\textcolor{blue}{where}": self, "\textcolor{blue}{sign}":">", "\textcolor{blue}{value}":150\}, }  
          \\
         \hspace{4mm}
          \texttt{\textcolor{blue}{association\_1\_2} := diagnosis = STEMI} 
          & \textcolor{gray}{7.} \hspace{24mm} \texttt{\{"\textcolor{blue}{where}": diagnosis, "\textcolor{blue}{sign}":"=", "\textcolor{blue}{value}": "STEMI"\}, }  \\
          \hspace{4mm} \texttt{\textcolor{blue}{pattern\_1\_1} := count} 
          & \textcolor{gray}{8.}
          \hspace{6mm} \texttt{"\textcolor{blue}{yaggregate}": ["count", "count"],} \\
           & \textcolor{gray}{9.}
          \hspace{6mm} \texttt{"\textcolor{blue}{ytype}": ["q", "q"],} \\
           & \textcolor{gray}{10.}
          \hspace{6mm} \texttt{"\textcolor{blue}{ylabel}": "Number of Records",} \\
          \hline
           & \textcolor{gray}{11.}
          \hspace{6mm}
          \cellcolor{yellow}{\texttt{"\textcolor{blue}{quantities}":[\{"\textcolor{blue}{name}": "ctb", }} \\
          & \textcolor{gray}{12.} 
          \hspace{15mm}\cellcolor{yellow}{\texttt{"\textcolor{blue}{filter}": \{"\textcolor{blue}{where}": self, "\textcolor{blue}{sign}": "<", "\textcolor{blue}{value}": 150 \},
          }}\\
          & \textcolor{gray}{13.} 
           \hspace{15mm}\cellcolor{yellow}{\texttt{"\textcolor{blue}{yaggregate}": "runningPercent"\}], }}\\
          & \textcolor{gray}{14.}
          \hspace{6mm}
          \cellcolor{yellow}{\texttt{"\textcolor{blue}{categories}":["type of admission", "patient district"], }} \\
          & \textcolor{gray}{15.}
          \hspace{6mm}
          \cellcolor{yellow}{\texttt{"\textcolor{blue}{times}": \{"\textcolor{blue}{monthly-annual}": ["pci"]\} }} \\
         

		 \hline
		
		\hline
	\end{tabular}
	
\end{table*}

Table~\ref{tab:mss} shows an example MSS for the \textit{Call-to-Balloon} metric, which matches the task structure specified in Table~\ref{tab:mort}.
The highlighted section of Table~\ref{tab:mss} pertains to subsidiary tasks; while
% (not supported in Vega-Lite)
lines $1-10$ parse the reference sets, associations and patterns specified for the entry-point task for this metric. In addition to tokens defined for the original task template, shown in Table~\ref{tab:templates}, this task defines two different ways to associate \texttt{\textcolor{blue}{reference(s)\_of\_set\_1}}. Namely, we expand \texttt{\textcolor{blue}{association\_1}} into \texttt{\textcolor{blue}{association\_1\_1}} and \texttt{\textcolor{blue}{association\_1\_2}}. This is to reflect that this task is the result of combining two tasks of the template \texttt{\textbf{BC1}}, as explained in Section~\ref{sub:wres}. 
%The first few lines of the MSS define the metric's name, the master task, a mark type to specify the preferred mark for this metric (based on experts' feedback), variable(s) used for the x-axis and variable(s) used for the y-axis and their data types.
%the $yaggregates$ amd $ylabel$ parameters specify an aggregation rule (e.g. sum, average, count, etc.) for each variable shown on the y-axis and an axis label, respectively. 
%At this point, the dashboard generation engine has everything it needs to generate the main view of this metric card. Note that this is structure is a simplified version of the view specification structures used in the Vega-Lite~\cite{satyanarayan2017vega}. 
%We avoid using visualization terminology (e.g. encoding, channel, etc.) to increase the accessibility of specifying MSS to users with basic technical knowledge, but we make no assumptions about their visualization background. 

In specifying these parameters for an MSS, dashboard administrators can decide what variables and aggregates are visualized on each axis for the main metric card view.
%This is because our engine does not allow as many degrees of freedom in the design space as the Vega-Lite grammar does. 
%In theory, the MSS can be expanded to add more flexibility to the individual view specifications. However, this is beyond the scope of this paper as our focus is on the adaptable generation of dashboard views based on the task structure obtained for each combination of audit, metric and user group. 
To specify subsidiary views to be shown in the expanded metric card, 
the MSS specifies three more parameters (highlighted lines $11-15$ in Table~\ref{tab:mss}): 
the {\tt quantities} parameter lists additional quantitative measures which are not already included in the entry-point task but possibly needed for subsidiary comparisons or associations (subsidiary task \texttt{ST1} in Section~\ref{sub:wres}). In the \textit{Call-to-Balloon} case, the additional quantities are: percentage of patients meeting target (see \texttt{TM3.1} in Table~\ref{tab:mort}) and average door-to-balloon time (\texttt{TM3.4}). 
 %We use the notation $der\_$ to show that a variable name that is specified in the MSS does not match any of the variables in the database. 
The {\tt categories} parameter lists nominal variables that are needed to answer subsidiary tasks which require a breakdown by category (\texttt{ST2} in Section~\ref{sub:wres}). 
In the \textit{Call-to-Balloon} metric, there are two such tasks involving two categorical variables: Method of admission (\texttt{TM3.2}), and patient district (\texttt{TM3.3}).

%The engine will lookup the derived variable name in a dictionary of derivation rules instead. In this specific case, the value of bed days is derived by calculating the difference between admission date and discharge date. 

The last parameter is {\tt times}; as time in itself is a referrer, we treat it differently in the MSS from the categorical and quantitative characteristics. 
Instead of a variable name, we specify a key-value pair (Line $15$ in Table~\ref{tab:mss}) which defines a time association rule (key) and a measure (value) exhibiting the pattern that the task aims to detect. 
For example, task \texttt{TM3.5} does not add any quantities or breakdown categories to the main question \texttt{TM3}. It inquires about the number of PCI patients, which is already part of the measures in the main task \texttt{TM3}.  
However, \texttt{TM3.5} adds a different granularity of time instances (years). In doing so, the question does not discard the original association (months) of \texttt{TM3}; it merely adds a second temporal granularity. 
In specifying two levels of granularity, we set an association rule \texttt{"monthly-annual"} as the key for an entry in the {\tt times} parameter, and the measure name {\tt "pci"} as the assigned value to this key. % to reflect that the task involves a comparison of months spanning different years.
Other tasks may drop the monthly association, in which case we use a single temporal granularity. For instance, if the task was comparing the current year versus previous years, we would set this entry as \texttt{\{"\textcolor{blue}{annual}": ["pci"]\}}. 
These parameters enable our dashboard generation engine to generate visualizations from a constrained design space. 
%In addition to the temporal association rule, we specify the target measure being addressed in the entry-point task. In this case, the task pertains to the number of PCI patients, for which the engine retrieves filters from the main view specification. 

%require the added time granularities as specified by the slave tasks. In this case, these characteristics are death in hospital (TM6) and admissions (TM7). 
% Given all of the parameters specified in the MSS as described so far, we explain how the dashboard engine parses them into visualization views and the design decisions made for each view in Section~\ref{sub:choices}.

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \begin{table*}[b!]
% 	\caption{Mapping the entry-point task in Table~\ref{tab:mort} and its subsidiary components to the corresponding Metric Specification Structure.}
% 	\label{tab:mss}
% 	\centering
% 	\scriptsize
	
% 	\begin{tabular}{|ll|}
% 		\hline
% 		\rowcolor{light-gray} \multicolumn{2}{|l|}{
% 		\texttt{\textbf{Task:} What is the number of delays and PCI admissions per month? }}  \\ 
% 		\hline
%  \rowcolor{lighter} AA Model Tokens & Metric Specification Structure(MSS)   \\
%  \hline
%          \hspace{4mm}\texttt{\textcolor{blue}{reference(s)\_of\_set\_2} := time of admission} & \textcolor{gray}{1.} \hspace{4mm} \texttt{\{"\textcolor{blue}{x}" : "date/time arrival at hospital",} \\
%          \hspace{4mm}
%           \texttt{\textcolor{blue}{association\_2} := months} & \textcolor{gray}{2.} \hspace{6mm} \texttt{"\textcolor{blue}{timeUnit}" : "month",}\\
%           & \textcolor{gray}{3.} \hspace{6mm}\texttt{"\textcolor{blue}{xtype}" : "temporal",}\\
%           & \textcolor{gray}{4.} \hspace{6mm}\texttt{"\textcolor{blue}{xlabel}" : "year",}\\
%           \hline
%          \hspace{4mm}
%           \texttt{\textcolor{blue}{reference(s)\_of\_set\_1} := patient admissions}
%           & \textcolor{gray}{5.}
%           \hspace{6mm} \texttt{"\textcolor{blue}{y}" : ["ctb", "pci"],}\\
%          \hspace{4mm}
%           \texttt{\textcolor{blue}{association\_1\_1} := delay > 150} 
%           & \textcolor{gray}{6.} \hspace{6mm} \texttt{"\textcolor{blue}{yfilters}" :[\{"\textcolor{blue}{where}": self, "\textcolor{blue}{sign}":">", "\textcolor{blue}{value}":150\}, }  
%           \\
%          \hspace{4mm}
%           \texttt{\textcolor{blue}{association\_1\_2} := diagnosis = STEMI} 
%           & \textcolor{gray}{7.} \hspace{24mm} \texttt{\{"\textcolor{blue}{where}": diagnosis, "\textcolor{blue}{sign}":"=", "\textcolor{blue}{value}": "STEMI"\}, }  \\
%           \hspace{4mm} \texttt{\textcolor{blue}{pattern\_1\_1} := count} 
%           & \textcolor{gray}{8.}
%           \hspace{6mm} \texttt{"\textcolor{blue}{yaggregate}": ["count", "count"],} \\
%           & \textcolor{gray}{9.}
%           \hspace{6mm} \texttt{"\textcolor{blue}{ytype}": ["q", "q"],} \\
%           \hline
%           & \textcolor{gray}{10.}
%           \hspace{6mm}
%           \cellcolor{yellow}{\texttt{"\textcolor{blue}{quantities}":["\textcolor{blue}{name}": "ctb", }} \\
%           & \textcolor{gray}{11.} 
%           \hspace{15mm}\cellcolor{yellow}{\texttt{"\textcolor{blue}{filter}": \{"\textcolor{blue}{where}": self, "\textcolor{blue}{sign}": "<", "\textcolor{blue}{value}": 150 \},
%           }}\\
%           & \textcolor{gray}{12.} 
%           \hspace{15mm}\cellcolor{yellow}{\texttt{"\textcolor{blue}{yaggregate}": "runningPercent"]\}, }}\\
%           & \textcolor{gray}{13.}
%           \hspace{6mm}
%           \cellcolor{yellow}{\texttt{"\textcolor{blue}{categories}":["type of admission", "patient district"], }} \\
%           & \textcolor{gray}{14}
%           \hspace{6mm}
%           \cellcolor{yellow}{\texttt{"\textcolor{blue}{times}": \{"\textcolor{blue}{monthly-annual}": ["pci"]\} }} \\
         

% 		 \hline
		
% 		\hline
% 	\end{tabular}
	
% \end{table*}


\begin{figure*}[tb]
 \centering 
 \includegraphics[width=\linewidth]{pictures/overview_edited.png}
 \caption{Minimized metric cards (left) and expanded view of the \textsl{Call-to-Balloon} card (right), showing an entry-point view with four subsidiary views.} 
 \label{fig:ctb}
 \vspace{-5mm}
\end{figure*}


==> tex/062_decisions.tex <==
Specifying metric cards through MSSs provides \textit{admin-level} adaptation that enables administrators to modify a dashboard's content to fit different datasets and contexts within their organization. Namely, through setting a minimalist set of parameters, they can specify for each metric card a main view that caters to the entry-point monitoring task, and sub-views to answer the initially known set of subsidiary tasks. Support for further subsidiary tasks is supported in the dashboard's Graphical User Interface (GUI) to support \textit{individual-level} adaptation. 
%while restricting customization decisions to be accessible to non-technical users.  
This section discusses design decisions that our dashboard generation engine makes at two levels of view hierarchy: the dashboard level and the metric card level.
We arrived at both sets of design decisions following a series of one-on-one meetings with four healthcare experts; three of whom had also participated in the co-design workshop. During these meetings, we showed the experts iterations of the dashboard generation engine in use and elicited their feedback. 

\bpstart{Dashboard-level design decisions}
%Our dashboard generation engine receives an array of MSSs as input.
% , where one metric care is generated for each MSS in the array. 
% The number of MSSs present in the array is equal to the number of metrics identified for each site. 
%Feeding new tasks and metrics to a dashboard means adding more MSSs to the input array. 
Given an array of MSSs, our dashboard generation engine dynamically generates corresponding metric cards for each MSS. 
Figure~\ref{fig:ctb}-left shows an example of a MINAP dashboard with four metric cards: \textit{Call-to-Balloon}, 
\textit{Mortality}, \textit{48-hour readmission} and \textit{Door-to-Angiogram}.
Double clicking a metric card expands it to show additional views that support subsidiary tasks relating to the metric (Figure~\ref{fig:ctb}(right)).

This idea of a \textit{``metric card''}~\cite{kaplan1992} as an enclosed view within the dashboard was inspired by the Balanced Scorecard (BSC), which is widely adopted in dashboards and typically uses enclosure to unite an organization's various perspectives into a consolidated view~\cite{pover}.
Metric cards are draggable, allowing users to prioritize the metrics that are most relevant to them.
They are positioned on the dashboard as a grid to avoid overlap, and users have control over how many cards are shown at any given time. Specifically, we allow users to toggle between \texttt{1x1}, \texttt{2x3}, and \texttt{2x2} layouts. Selecting the \texttt{1x1} layout expands all cards and allows the user to scroll vertically through them as one would a PDF slide presentation.
% while the other two layouts create \texttt{2x3} and \texttt{2x2} tiles, respectively. 

We first introduced our stakeholders to the idea of a \textit{Metric Bubble}, inspired by Code Bubbles~\cite{bragdon2010code} and VisBubbles~\cite{li2011visbubbles}, as an enclosed view that allows flexible dragging and resizing.
The idea was well-received. However, the free dragging and resizing behaviour for the bubbles was perceived as overwhelming and allowing \textit{``too many alternatives''} by our domain experts. 
They argued for a more restricted dragging mechanism for laying out and resizing the metric enclosures on the screen. 
In response, we considered two layout options: a tabbed view that displays each metric card on an individual tab and a grid layout that places them on a single screen in a tiled manner. 
Empirical evidence shows that juxtaposed
patches on a grid layout significantly reduces navigation mistakes over tabbed views~\cite{henley2017toward}. While this finding was observed in the context of code editors, we believe that the transition between examining different code fragments bears some similarity to the process of proceeding from one metric to another. 
We therefore allow users to drag to reposition cards; when expanding a card, other cards are also repositioned.
%  

\bpstart{Metric-card-level design choices}
\label{sub:main}
Each metric card initially displays a single bar chart that addresses the entry-point task for the corresponding metric. 
%Additionally, the engine creates three hidden sub-views for each metric card. 
The choice of a bar chart is motivated by the very nature of the task structure for entry-point tasks, which predominantly follow the template \texttt{\textbf{BC1}} (see Table~\ref{tab:templates}).
It also matches the expectations of our stakeholders as collected through co-design activities (See Figure~\ref{fig:activ1}) and our one-on-one meetings with experts. 
The use of MSSs to specify the cards allows for future expansions to support other chart types via adopting a \texttt{mark} operator from the Vega-Lite grammar. 
%However, for the sake of compactness we default all views to the \texttt{rect} mark type which is enough for entry-point tasks.
For \textit{admin-level} adaptation, we specify the mark type for each of the views, and allow administrators to tweak data and aggregation rules for each view. 
Furthermore, the MSS makes a few design choices for the main view of a metric card. 
First, the engine considers the number of measurements assigned to the y-axis. % as specified by the \texttt{"y"} parameter. 
If the number of measurements is less than a threshold $\tau$, it draws a grouped bar chart to present the measures. 
If a larger number of variables is assigned to \texttt{"y"}, the engine will instead produce a small multiples view as entry point view. 
Furthermore, an optional parameter \texttt{"chartType"} allows dashboard authors to override view defaults and specify either a \texttt{"stacked}, \texttt{"grouped"}, or \texttt{"small multiples"} view for the main card view.  

%The Mortality, Bed Days and 48h Readmission cards in Figure~\ref{fig:dashMain}are examples of this category. If the number of measurements is between $\tau$ and another threshold $\Upsilon$ the engine opts for stacked bars instead.  
%The Dependency card (TODO: reproduce after fix) in Figure~\ref{fig:dashMain} is an example of this category. We currently set $\tau = 4$ and $\Upsilon=8$. Any number of measurements larger than $\Upsilon$ will direct the
%engine to create a trellis view. The Case mix metric card in Figure~\ref{fig:dashMain} shows an example. 
%Users can override these default views by toggling between the three views. 

Views supporting subsidiary tasks become visible only when a card is expanded.
The three subsidiary views shown in Figure~\ref{fig:ctb}(b), (c) and (d) correspond to the three types of measures defined in the MSS:  \texttt{quantities}, \texttt{categories} and \texttt{times} parameters. 
Since each of these types may contain more than one measure, each subsidiary view generates a number of tabs that is equivalent to the number of variables assigned to each parameter. For example, view (c) in Figure~\ref{fig:ctb} has two tabs for {\tt "type of admission"} and {\tt "patient district"} measures specified in the {\tt categories} parameter of Table~\ref{tab:mss}.
%TODO: add in this section the discussion of positioning  historic data in a sub-view

Also informing the choice of visualization in the entry point view is the \texttt{yaggregates} parameter. 
%The choice of bar chart according to the rules described above only applies if the elements of the $yaggregates$ array are all the same. 
When different aggregates are listed for this parameter (e.g. \texttt{count} and \texttt{percentage}), this indicates different scales. 
In such cases, we designed our visualization engine to generate
a dual axis and a line overlay on the bar chart to represent measures with different scales.
While empirical evidence recommends against the use of super-imposed dual-scale 
charts for comparison tasks~\cite{aigner, 6065014}, these recommendations are specific to dual scales with the same mark encoding. It is less clear how people perceive differences with different mark types assigned to different scales. 
Furthermore,
our entry point tasks do not involve comparisons between the different scales. Instead, they constitute combinations of behaviour characterization (i.e. direct lookup) tasks. Andrienko and Andrienko argued that in this class of tasks \textit{"it is possible to consider
any attribute independently of the other attributes"}~\cite{andrienko2006exploratory}. We use this argument to justify our choice of line overlays in tasks like \texttt{"What is the raw number of deaths and the standardised mortality ratio (SMR) per month?" } where raw counts can be visualized as bars and SMR as a line overlay. 
% While a user may want to see the raw counts on a bar chart, they can monitor SMR with a line overlay. %Alternatively, they can opt to separate SMR from the main view and include it as part of the \texttt{quantities} sub-view.  
%This choice between an entry-point view and a subsidiary view is governed by the urgency of each measure within each site. 

%If more than two aggregates are listed, only two are used in the main view and additional aggregates (and their corresponding measurements) are added as a tab in the $quantities$ sub-view. 

Figure~\ref{fig:ctb}(b) shows an example {\tt quantities} subsidiary view. While serving a similar purpose to the entry point view (i.e., plot one or more measures over time), we use similar design choices for this subsidiary view. Therefore, each measure in the \texttt{quantities} array has its own  \texttt{name}, \texttt{filter} to specify which records should be included in this measure, and an aggregation rule ($yaggregate$) to specify how monthly aggregates are calculated. 
To visually distinguish categorical from quantitative measures, we use a pie chart for measures listed in the \texttt{categories} array of the MSS. 
Our use of pie charts for this sub-view is motivated by two factors: 
\textit{(i)} a need to distinguish their nominal domain from the temporal domain for which the other views in the metric card use bar charts; and
\textit{(ii)} the prevalence of pie chart use in healthcare quality improvement reports which increases users' familiarity with the dashboard. 
To avoid creating tabs that are too small, we limit the number of tabs for any subsidiary view to four variables. Buttons on the right side of each subsidiary view toggles a popover element that contains a full list of variables of the same type. 
For example, the popover menu shown in Figure~\ref{fig:ctb}(e) enables users select alternative \texttt{quantities}. 
%Through these multiselect lists, users can modify the group of variables being included. Once they update their selection of variables, a new list of tabs gets populated. 

The \texttt{times} subsidiary view creates tabs for each key-value combination listed in the \texttt{times} MSS parameter.  
Since we consistently treat time as a referrer in our task model, the structure of elements in the \texttt{times} MSS parameter is inherently different from the structures described thus far, as explained in Section~\ref{sub:mss}. 
%Specifically, we use a key-value combination for each element in the array. The key is composed of one or more time granularities and the value is the variable name that needs to be shown at the corresponding granularities. In the examples shown in Figure~\ref{}
For tasks with a mixed temporal association (e.g. \texttt{TM3.5} in Table~\ref{tab:mort}), we specify a small multiples view, in which the first association is used to segment the second. The example shown in Figure~\ref{fig:ctb}(d) displays annual comparisons segmented by months. We further enable users to toggle between this view and a multi-series line chart. 
%Due to the nature of entry-point tasks, we do not support time frame selection in our GUI. This is to prevent a user from accidentally selecting an outdated dataset for monitoring purposes. On the other hand, we support investigation of historic data through restricting the display in the \texttt{times} subsidiary view.  

Subsidiary views in a metric card are linked to the entry-point view.
For example, brushing a pie chart in a \texttt{categories} subsidiary view will highlight the distribution of the corresponding category over time in the entry point view. The converse is also true, in that brushing a month in the bar chart causes the pie chart to update and display the distribution of the categories within the brushed month; this brushing also highlights the corresponding month in the \texttt{quantities} view.
% The expanded \textit{Call-to-Balloon} card shown in Figure~\ref{fig:ctb} answers the task \texttt{TM3.1}, \texttt{TM3.2} and \texttt{TM3.5} from Table~\ref{tab:mort}.
Consider the expanded metric card shown in Figure~\ref{fig:ctb} (right); by highlighting a month with a relatively high number of delayed patients (April), one can see that 50\% of these patients self-presented to the hospital, 25\% were recovering after a PCI procedure, and 25\% were already in the hospital. Given this finding, a user can exclude external factors (from indirect admissions) that may have caused these delays for at least 50\% of the cases in April (\texttt{TM3.2}). Simultaneously, the same month is emphasized in the \texttt{quantities} subsidiary view, which displays monthly percentages of patients who did in fact meet the target (\texttt{TM3.1}). \texttt{times} subsidiary view compares each month to the same month in a previous year (\texttt{TM3.5}). Finally, other tasks pertaining to this metric are addressed by switching from one tab to another in the subsidiary views.    

\bpstart{Implementation} We implemented the metric cards in HTML and made use of Muuri.js~\cite{muuri} to maintain forces between cards and  allow a responsive shuffling behaviour when cards are dragged or expanded. We use D3.js to generate the visualizations in each view.% We make our dashboard engine available as open-source. The source code can be downloaded at ({\tt \underline{link removed to preserve anonymity}}). 


==> tex/08_validation.tex <==
We validated the TASHA workflow by evaluating the resulting dashboard designs for the MINAP and PICANet audits.
We conducted three focus group sessions with healthcare professionals from three hospitals, during which we focused on answering questions relating to how the tasks we sampled are supported by the dashboard designs. 
Specifically we wanted to answer the questions:
\textit{Q1:} Do the metric cards capture the \textit{structure} of the relevant tasks for each site? (stages \textit{(a)} to \textit{(d)} in Figure~\ref{fig:flow}),
%\textit{(ii)}  Does the choice of data variables, visualizations and interactions in a metric card support relevant task sequences? 
 %\textit{Q2:} Does the level of customization supported in the metric cards offer good usability for currently supported metrics? 
 \textit{Q2:} Can we expand the dashboard to add new metrics as they arise? (stage \textit{(e)} in Figure~\ref{fig:flow}), and finally \textit{Q3:} How usable is the dashboard? The latter question aims to inform a training plan while anticipating the dashboards' use in the sites. 
%and \textit{Q3:} For customization involving , can we efficiently add new cards that supports them? 
%Finally, we also aimed to test the usability of the interface and develop a training plan anticipating the dashboards' use in the sites. 

The first session featured an \textit{active intervention with a paper prototype}~\cite{lloyd}. 
Participants were divided into three groups.
% (see Figure~\ref{fig:codesign2} left). 
Each group was handed prototype material for a set of metric cards. 
% (Figure~\ref{fig:codesign2} right).  
For each metric card, the paper prototype included: a task that we believed to be of high relevance, based on stages \textit{(a)} to \textit{(d)} of the TASHA workflow as illustrated in Figure~\ref{fig:flow}, 
screen printouts of metric card(s) that address the task, and a list of database variables that were used in the construction of MSSs used to generate the cards, based on stage \textbf{(e)} of the workflow. 
Appendix C in our supplementary material shows some of these example metric card printouts. 
%In cases where a task can be performed in more than one way (e.g. by including different metric cards or different variables), we printed out all alternatives and asked participants to reflect on them. 
We encouraged participants to rephrase or change a task if it was not addressing a priority for the participants' site, to comment on the data elements used, and to sketch ideas to improve the visualizations shown on each metric card.
The aim of this session was to set the focus on 
%We discuss the results of analyzing the notes and sketches from this session in Section~\ref{sub:evalres}
%Five data-related issues were raised by participants during this session. Primarily having to do with the way some variables are calculated. For example, for 

Later, two sessions featured a \textit{think-aloud protocol}~\cite{rogers2011interaction} with participants in two sites.
In each session, we divided participants into groups, where each group consisted of 1-2 participants and a facilitator using one computer to interact with the dashboard. The facilitators gave a short demo of the prototype. 
% Following this, participants in each group took turns interacting with it and practicing the think-aloud protocol.
As an initial training exercise, the facilitator asked participants to reproduce a screen which was printed on paper. 
This reproduction exercise was intended to familiarize participants with the dashboard and the think-aloud protocol. 
Following this step, the facilitators presented a sequence of tasks to participants and observed how they interacted with the dashboard to perform these tasks. 
We captured group interactions with video and audio recordings in one of the sessions, and recorded the screen along with audio in another. 
%We recorded both video and audio from these sessions.
%We summarize our findings from analyzing the recordings and the facilitators' notes in Section~\ref{sub:evalsub}.
In addition to collecting qualitative feedback, we also administered a System Usability Scale (SUS) questionnaire~\cite{brooke1996sus} at the end of each think-aloud session. We asked participants to complete the questionnaire after an hour-long interaction session with the dashboards. 
%We elicited further feedback through additional meetings in three hospitals and followed up by email, during which a demo of the dashboards was presented by a team member, followed by a discussion. 
%A description of the analysis of results for all sessions follows.

% \begin{figure}[tb]
%  \centering 
%  \includegraphics[width=.47\linewidth]{pictures/IMG_1924.jpg}
%  \includegraphics[width=.47\linewidth]{pictures/IMG_1928.jpg}
%  \caption{Active intervention session with paper prototype was attended by seven healthcare professionals and facilitated by four team members.} 
%  \label{fig:codesign2}
%  \vspace{-5mm}
% \end{figure}

% \subsection{Analysis of Results}
% \label{sub:evalres}




%TODO: Need to explain in total how many participants? Seven healthcare professionals participated in these two sessions including a cardiologist, an information manager, a PICU consultant, an audit coordinator, two clinical effectiveness and compliance managers and a nurse. Four of our team members facilitated the sessions. 
\bpstart{Results}
Seventeen healthcare professionals participated in these focus sessions, which included cardiologists, information managers, PICU consultants, and nurses, among other professions. 
We analyzed the sketches, observation notes, and recordings from all sessions and divided participants' feedback into six categories: 

\begin{itemize}[noitemsep,nolistsep,leftmargin=*]
    \item A \textit{task-related} category captured the (mis)match between participants' intended questions and ones that are currently supported by the dashboard. 
    \item A \textit{sequence-related} category captured comments relating to the (mis)match between the structure of the views and participants' intended task sequences. 
    \item A \textit{data-related} feedback category captured comments relating to the data variables in the MSSs used to generate the metric cards. 
    \item A \textit{visualization-related} category 
    captured feedback on the choice of visual encodings in each view. 
    \item A \textit{GUI-related} category attended to comments made on the graphical interface elements, not related to the visualizations.
    \item A \textit{``Other''} category reported any further comments. 
\end{itemize}

Example instances from each category are included in the supplementary material (Appendix B). 
The paper prototype session  aimed to free participants from learning a new software and rather set the focus on the match between the tasks, data and visualizations on one end and participants' needs and expectations on another (\textit{Q1}). The think-aloud sessions focused on assessing the expandability (\textit{Q2}) and usability (\textit{Q3}) of the dashboards. 

In answering \textit{Q1}, we collected a total of 12 data-related suggestions; of which 6 suggestions were readily supported by modifying the parameters of the MSS. For example, comments like \textit{``PIM score aggregate can be average or mode, but not sum.''} were immediately addressed by changing the MSS parameter \texttt{yaggregate} for this measure. 
Other suggestions were addressed through further development iterations to allow more flexible data aggregation. For example, we added two more aggregation rules \texttt{cumulativeSum} and \texttt{cumulativeAverage} to address comments like \textit{``SMR should be looked at as a cumulative value rather than a monthly average because our performance is judged on it annually, so we want to know how we are doing so far''}.
%On the task-related front, participants' comments were generally very positive. 
%We recorded several data-related items of feedback. For example, rather than displaying unplanned extubations as a raw number, participants indicated that they would prefer to see it as a percentage of total invasive ventilation events. 

On the task and sequence-related fronts, participants commented positively on the match between the dashboard and their thinking process. 
%One participant commented that \textit{``one could make a fortune with this!''}. 
A participant group, for example, attempted to answer the question \textit{``What is the case mix for deceased patients in April?''} 
They approached the task with two different sequences: first by identifying deceased patients in April and examining the percentage of different diagnoses in this group; and then by reversing the sequence and highlighting patients of a specific diagnosis to see whether they could reach the same answer.  
One participant commented \textit{``People approaching the visualization with different questions will view consistent data subsets and that’s good''}. 
%People will try different things but they’re getting the same answer so that makes it a foolproof mechanism''}. 
We also recorded four task-related adaptation items. Namely, to accommodate new metrics that arose from the discussion and were not collected the interviews (e.g. percentage of patients given gold standard drugs). 
We found that these newly emerging tasks followed the same structure of our identified entry-point tasks and led to subsidiary tasks that followed the same patterns defined in Section~\ref{sub:wres}. 
We were able to generate alternative metric cards for those sites by specifying new MSSs, which answered questions \textit{Q1} and \textit{Q2} of our evaluation. 

Furthermore, we collected 21 visualization and GUI-related comments, including positive feedback and a few suggestions to include overlays showing target lines where metrics are meant to achieve a nationally defined target.
We plan to add functionality to support these overlays before we release the dashboards into the sites in June 2019. Overall, participants had a very positive response toward the dashboards and the prospect for integrating them into their practice. 
%As an example, one participant commented \textit{``What I want to see is a line with the percentage of mortality out of raw admissions to then be able to compare across months''}.
%In visualization-related comments, we addressed comments that requested overlays to be included on the bar charts, and restricted the sub-views to avoid showing the same information displayed in the main views. 
%Sequence-related comments were also positive. One participant said: \textit{``It’s good to have the SMR and PIM scores in the bar sub-view because it tells you how sick the cohort was''}.
%A mismatch arose with the sequence of tasks for the smaller sites which did not measure some of the metrics that were displayed in the main views and instead requested to move these metrics from the sub-views up the hierarchy to be displayed in the main views. 
%We modified the MSSs for these sites to reflect this change. 
Finally, the usability feedback was largely positive save for minor issues (e.g., legend position, size of labels, etc.). 
% Otherwise, participants commented positively on the usability of the dashboards.
Usability scores from the two think-aloud participant groups were 74 in the first session and 89.5 in the second session, which indicates very good usability (\textit{Q3}). 

%Of specific interest to us was the question \textit{‘I needed to learn a lot of things before I could get going with this system.’} which had the lowest score; participants mostly disagreed with this statement. One participant commented: \textit{``this would only be in relation to the datasets being uploaded.''}


%Indeed, participants who were familiar with audit data were most comfortable answering the questions. Participants who had little familiarity with what the variables in the data mean (e.g. what is ``call-to-balloon'') felt that they needed more information about the meanings of the variables. However, once data meanings were clarified for these participants, understanding the visualizations and interactions supported came naturally with no further support needed. One participant commented  

% \subsection{Limitations and Future Work}
% The vast majority of limitations found through our discussions with stakeholders had to do with the varying abilities of different users to understand the scope and definition of variables in the data. 
% Participants with average-to-high familiarity with the audit data were able to use the dashboard fluently and understand what they were looking at, while participants who had no previous exposure to audit data struggled to understand variable names in customization elements.
% Moreover, some participants noted that lack of familiarity with the data can lead to different interpretations. For example, while someone familiar with MINAP data would know that ``door-to-angio'' means the time between admission and an angiogram, while someone with less familiarity may interpret it as angioplasty or may not be sure what the visualization is displaying. 
% To rectify this issue, we will link data definition manuals to the dashboards. 

% Another limitation arises from data quality. Gschwandtner et al.~\cite{gschwandtner2012taxonomy} presented a taxonomy of data quality problems in time-oriented data. 
% TODO: connect this next bit to the taxonomy.
% Despite that our dashboards show data retrieved from the audit after its validation, there are still many concerns around the data entry process and missing values in the data. 
% To address this limitation, we display data completeness information on a per-variable basis in a visualization's legend (Figure~\ref{fig:expand}), but we acknowledge that this solution is not ideal. We initially proposed adding a metric card for data quality, however this idea was not well received, as participants said they would prefer to see data quality information incorporated in each card rather than in a separate card. 
% As we expand the TASHA workflow in our future work, we will explore the possibility of adding a parallel track through the workflow that analyze users' needs not only with respect to data understanding but also with respect to the level of trust and uncertainty in the data. 


%1. workshop
%2. focus groups
%3. feedback: 
%Data-related, visualization- related, GUI-related, interaction-related, new-related + training and adoption-related 
%(No need for training sessions (a few minutes of demo is enough) + IT training  troubleshooting + data loading 
%Awareness + introduce it to ppl (not training) 
%End users Confident about the interpretation of the visualization (what data is shown and how). 

%First round of evaluation The average score was 74 out of a 100 (where 80 signifies very good usability), 
 

%They say with the SUS you shouldn’t look at scores for individual questions but only look at the overall score. However, I couldn’t help noticing that the lowest scores were for the question ‘I needed to learn a lot of things before I could get going with this system.’ One participant added a comment that ‘this would only be in relation to the datasets being used.’ Interestingly, understanding the data (understanding what different variables represent, as opposed to understanding the visualisations) was a topic that came up yesterday in the adoption workshop – so a topic worth discussing, in terms of design and/or training, in our meeting tomorrow.

%Second round: SUS Score from 89.5 – so very good usability

==> tex/algo.tex <==
The reasoning procedure about the set of master-slave tasks then proceeds as follows: 
	For a master task that involves a “trend” as a member of its “target” vector:
	The program begins by finding the temporal variable in this task’s variables vector, and assigns this variable to the x-axis of the master view.
	The program then looks for the population granularity of the task:
	If the granularity is an aggregate (e.g. count, average, etc.), then the program sets “bar” as a default mark type. Then looks for temporal granularity to create either daily, weekly, monthly or annual aggregates. 
	If the granularity is “individual” then the program sets “line” as a default mark type and looks for the temporal granularity to set the scale for the x-axis.
	In cases where granularity is a composition of different levels, the coarser level is appended to the variable list as nominal. For example, the task “Is mortality rate this January higher or lower than the same month last year?”  has a granT vector [“monthly”, “annual”]. In this case, the “monthly” level is used for the time dimension while the “annual” level gets treated as a nominal. 
Note that these default choices can be modified by user actions. 
	The program then creates a list of unique criterion variables that are obtained from the non-temporal elements of the variable vectors for the master task and all of its children with “ISA” links to the master. The variable types in this list are examined: 
	Quantitative variables are binned and treated as ordinal variables
	Selection of bar grouping variable(s): 
	The first occurrence of a nominal or ordinal variable is used as a grouping variable
	The second occurrence is used as a stacking variable
	Any remaining variables are added to a queue (for interactive addition/removal of grouping variables) 
	A saturated visualization for a master task has data variables assigned to the following visual components:
	X-axis
	Y-axis
	Grouping 
	Stacking 
	If the master visualization for a metric is not saturated yet (e.g. if it has a grouping variable but not a stacking variable), then it can take a variable from one of the slave tasks. 
	

	For a master task that does not involve a “trend” as a member of its “target” vector:  


==> tex/algo2.tex <==
In specifying the views for a dashboard, we introduce the notion of a MetricView, a self-contained area of the dashboard that contains all pieces of information pertaining to a specific healthcare quality metric. 
The metric view is divided into a main view, which caters to the master task of this metric, and a set of slave views that cover ``grouping'', ``comparisons'', ``benchmarking'' and ``detail'' tasks, respectively. 
Figure~\ref{fig:metricView} depicts these different components of the MetricView. 

In this manner, a dashboard is viewed as a two-level hierarchy of visualization composition: At the lowest level, a visualization view caters to one or more user tasks.
Individual Views occupy one of the five different areas of a MetricVew, which constitutes the middle level of the hierarchy. 
Finally, at the top level of the hierarchy, a composition of MetricView's forms the entire dashboard. 

This intermediate level of information composition (between a single view and a dashboard) simplifies the problem of dashboard design and constrains the design space in a manner that makes the process amenable to automation. 
Namely, to accommodate the great diversity of metrics and user tasks for individual audits, the views of the dashboard are dynamically generated from a view specification data structure.
This data structure is automatically generated from the task specification grammar described in~\ref{sec:codesign}. 
It is then mapped to a view specification data structure that specifies the data and visualizations that fit in each of the views
that contains the following elements:
\begin{itemize}
    \item Metric: is a metric name that displays the title of the MetricView and pulls a JSON file that contains descriptions of derived variables (if any) that are used for this metric.
    \item mark: similar to Vega-lite grammar, the mark specifies what mark type is used by default for the main view. 
    \item x and y: specify one variable that goes on the x-axis of the main view and up to two variables for the y-axis
    \item scales: describe the scales of all variables per axes. This is to make decision, for example, about adding a dual axis to a bar chart if the y-axis is showing two variables with different scales. 
    \item Categories: contains grouping categorical variables that are typically used to split the data shown for this metric.
    \item Comparators: visualizes variables and external data entities that are used for comparison
    \item Benchmarks: lists all the possible overlays that could potentially be 
    \item Detail: 
\end{itemize}


==> tex/eval.tex <==
MAIN CONTRIBUTION: EVALUATION STRATEGY TO MAKE EFFICIENT USE OF LIMITED CONTACT TIMES WHILE ENSURING A ROBUST SYSTEM. 

Table~\ref{tab:eval} provides an overview of these activities.  

\begin{table}[h]
% 	\vspace{-5mm}
	\caption{QualDash evaluation activities}
	\label{tab:eval}
	\centering
	\scriptsize
	\begin{tabular}{|c|c|c|}
		\hline
		  & \textbf{On-site} & \textbf{Off-site} \\
		  \hline
		  \textbf{Insight} & Focus groups &  Think aloud protocol \\
		  \hline
		  \textbf{Usability} & Testing protocol  &  Heuristic evaluation \\
		  & & and SUS Questionnaire \\ 
		  
	    \hline
	\end{tabular}
	
\end{table}
\subsection{Insight Acquisition}
\label{sub:valid}

\subsubsection{On-site evaluation}

\subsubsection{Off-site evaluation}

\subsection{Usability Testing}
The purpose of our usability testing was to capture issues that presented challenges to the usability of the interface of the dashboards. Testing was primarily focused on the Graphical User Interface (GUI) features of the web tool, navigation within and across QualCards and functions like exporting selections to tabular view, exporting and downloading visualization views and raw data, adding and removing tabs in the QualCard subviews, etc. 
Off-site usability testing was done via heuristic evaluation by four domain experts and on-site testing was performed by two of our team members from a healthcare background. Details of our findings from both analyses are provided here. 

\subsubsection{Off-site Usability Testing}
Four domain experts performed a heuristic evaluation of the dashboard interface: a freelance data visualisation specialist with over 10 years experience as a consultant, training provider and author, a clinical professor of primary care with 20 years experience with clinical audit evaluation and implementation research, and two Human-Computer Interaction (HCI) researchers with 10-15 years in clinical informatics research. 
To support this evaluation, a mock dashboard was published using simulated data on a public hosting site. 
Each expert was provided with a link to access the simulated dashboard and a questionnaire to fill about it. 
Appendix XXX includes a sample of the questionnaire.



In addition to heuristic evaluation, we administered a Software Usability Score (SUS) questionnaire at the end of the workshop described in Section~\ref{sub:valid}

\subsubsection{On-site Usability Testing}
Two team members from a healthcare background performed the on-site usability testing. These team members were not involved in the development of QualDash. They, therefore, regarded the tool from an end-user's perspective. 








==> tex/formal.tex <==
The input for the TASHA framework is a corpus of tasks that are collected through interviews and other qualitative methods. 
In the case of dashboards, the task space is typically very large due to the vast diversity of user types and interests, as noted in~\cite{}. 
Our project team has conducted a total of 56 interviews with different healthcare professionals to gain an understanding of their usage of clinical audit data and their vision for a dashboard that could help their decision making for healthcare quality improvement.
The first phase of our task analysis was then to go through the transcripts of these 56 interviews while digging for user tasks (i.e. questions that participants showed interest in answering from the data). 
A total of 124 questions were collected in this initial phase. 
This number grew as the number of interviewed participants increased. 

One notable observation is that many of the tasks were in actuality inquiring about similar data constructs. However, when stated in natural language, they were stated differently by different interviewees. 
A systematic approach was needed to dissect the collected tasks and  map them from their natural language format to a structured task feature vector, to enable reasoning and clustering. 
In this section, we present a systematic approach to position tasks collected in natural language along different dimensions of the task space, and to sample the space to produce a more manageable group of abstract tasks. 
The components of a grammatical specification of a task include the following: 
\begin{itemize}
    \item A $\mathbf{task}$ phrase: this is the textual representation of the task. 
    \item $\mathbf{variables}$ and $\mathbf{vtypes}$ vectors: list the database variables that should be fed to the visualization (along with any formulae that should be applied for derived variables) and the corresponding data types ($\mathbf{n}$: nominal, $\mathbf{q}$: quantitative, $\mathbf{t}$: temporal, $\mathbf{o}$: ordinal).
    \item $\mathbf{aggregates}$ a vector specifying the roles of the different variables in the task and the effect the variable will have on the presented data elements. Levels for this feature include aggregate functions (e.g. count, average, etc.), temporal units (e.g. day, month, etc.) and variable roles (e.g. group, filter). 
    \item $\mathbf{target}$ a vector specifying the target information that could be delivered by the variable (as specifiec in ~\cite{BELIV}. 
\end{itemize}

Contrast to~\cite{BELIV}, in which a single target was specified for a given task, we specify a target for each individual variable. We have found this to be more descriptive of the role of each variable in a task, as will be shown by the examples in this section.
%In the example in Figure~\ref{fig:grammar}, the time variable specifies the trend, the aggregate count helps identify the objects that (do not) meet specific criteria, and the two nominal variables display the proportion of the records meeting the main criterion (i.e. patients who experienced delays in their call-to-balloon time), and the proportion of different patient sub-groups (STEMI, nSTEMI).  Notice that the proportion target is repeated twice in this vector to indicate that a two-variable grouping is required for this task. 
%In addition to this variable-target mapping, a vector $\mathbf{vroles}$ keeps track of which variables are input to a task and which are targeted as output. In this example, the nominal criterion is the only output. All other variables are given as input. 
%To fill the $\mathbf{granP}$ and $\mathbf{granT}$ entries for this task, we simply asked participants to specify the time granularity and patient data granularity that would be required to give the information targets by a task. For the example task in Figure~\ref{fig:grammar}, participants have specified in their answers that this metric should be monitored on a monthly basis at the unit level. Therefore, we assign these values for the $\mathbf{granT}$ and $\mathbf{granP}$ entries. 
%Since questions in the task sequence are collected from participants in natural language, we sought a systematic approach in order to extract the different data components from each task. This step is to guide the mapping between collected tasks and the task grammar, which was detailed in Section~\ref{sub:grammar}. 

To obtain the desired structure from task wording, we created a corpus of question types from the different taxonomic categories described systematically by Andrienko and Andeienko in~\cite{andrienko_book_chapter_3}.
[TODO: explain some rationale here on why we chose the AA model for this step]. 

 An initial list of question templates is curated by examining the analysis task examples from the AA book. This list is subject to expansion as more questions are phrased in different ways by interview and workshop participants. This list is, therefore, not exhaustive but aims to provide some guidelines that help analysts reason about tasks and the way each referential component/characteristic is treated when mapping a task from its original form in natural language to a corresponding feature vector. 
 A table listing the different task templates can be found in Appendix A (See supplementary material).   
Questions expressed in natural language are tokenized using their corresponding data model components.
Additional elements that are external to the data model (e.g. benchmarks) are annotated between square brackets. We refer to the abstract tokenized form of a task as a``task template''. 

It is worth noting here that our consideration of the phrasing of a question provides a detailed specification of the task classes specified in the in AA model. For example, lookup tasks can be further specified as: simple lookups and criteria-matching lookups. 
Examples of simple lookups include:
\begin{itemize}
\item \textit{``T1:What is the raw death count and the risk-adjusted SMR per month?''}
\item \textit{``T2:What is the number of discharges per month and the proportion of these that were readmitted within 48 hours?''}
\end{itemize}
These examples follow the task template 
\textbf{TEDL1: What is/are the $<characteristic(s)>$ of $<reference(s)>X$?}
and make clear that users are seeking to understand the values of the output characteristic. They may wish to monitor the change in these values over time or their distribution across different groupings. 

Mapping this type of tasks to the corresponding feature vector is as simple as identifying the $<reference(s)>X$ and $<characteristic(s)>$ components and specifying the data types, granularity and targets for these components. 
For the example T1 above, $<reference(s)>X = \{time\}$. The granularity for which is defined by a feature granT, which in this case is a month. 
Therefore, we append a temporal variable to the task's $variables$ vector. We specify its data type in the $vtypes$ vector.
%Both variables are input to the task so their corresponding %$\mathbf{vroles}$ are ``in''. 
The target of this first variable can be either specified as a trend over time or a distribution. 
In TASHA, a trend variable would result in a visualization that shows time as a continuum (e.g. using line or area marks). 
We use the ``distribution'' target to specify more discrete temporal patterns. 
This distinction can be inferred from the phrasing of the task.
 %a distribution of the calculated aggregate over different referrer sets (in this case months). 

%This partial specification, if put in a vega-specification format, would potentially lead a visualization recommendation tool like Draco to display the temporal variable on the x-axis and the quantitative variable on the y-axis. However, it is not clear at this point what exactly the y-axis should represent. Is it a count of all records that occurred in the corresponding months? or is the user interested in counting specific values for the characteristic(s) of interest?
The vector $<characteristic(s)> = \{death, SMR \}$ includes two characteristic variables. Therefore two variables will be appended to the list of variables for this task: $unitDisStatus$ is a nominal database variable that stores the discharge status of a patient (alive or dead), and $SMR$ (Standardised Mortality Ratio) is a derived quantity that can be calculated at the desired (monthly) referrer granularity.
The target for the $unitDisStatus$ variable is to display a specific value ``dead'', and the $\mathbf{SMR}$ variable aims to show a distribution of values calculated by the sum of SMR for each aptient. 
%These two characteristic variables are targeted as output by the task, therefore their roles are assigned as ``out''. 
At this point, the task T1 has the following feature vectors: 
$\mathbf{variables}: [time, unitDisStatus, SMR]$, 
$\mathbf{aggregates}: [month, count, sum]$,
%$\mathbf{vtypes}: [t, q, n, q]$ 
%$\mathbf{vroles}: [in, in, out, out]$, 
$\mathbf{targets}: [distribution, value, distribution]$. 

Notice that the type cardinality of a task can be inferred from the specification given so far. For example, through looking at the the aggregates vector, one can see that the first variable is a temporal one and that the other two variables are quantitative. 


%We begin by mapping an input task to the most similar task template in the table. This matching is currently done manually, but could potentially be aided with NLP techniques. TODO: like what?

In contrast to simple lookup tasks described thus far, criteria matching tasks can be phrases in a more subtle manner. [TODO: Distinguish here between criteria matching with specific values like this versus when the ctieria has a range (e.g. danger zone) in which case the additional variables are quantitaitve ranges]
%Matching a task to its template in this fashion facilitates the reasoning about the components of the task and the role of each variable, and the information being targeted. 
For example, many of the collected tasks involve monitoring a metric over time.
Examples of these tasks include:
\begin{itemize}
\item \textit{``T3: Does the call-to-balloon time for STEMI/ nSTEMI patients meet the national target?''}, and \item \textit{``T4: Did the length of stay for cardiac patients exceed the expected duration?''}.  
\end{itemize}
Note that, when phrasing these questions, the participants did not specifically mention time. 
%We used the 3D task space specified in ~\cite{BELIV} to structure further communication with participants. 
Therefore, when asked to specify the time granularity at which they would like to monitor these metrics, they specified a monthly level. Therefore, an analyst-expanded version of the tasks above might read: 
\textit{``T3*: For a given period of months, does the call-to-balloon time for STEMI/ nSTEMI patients meet the national target?''}, and 
\textit{``T4*: For a given period of months, did the length of stay of cardiac patients exceed the expected duration?''}
This latter format can be mapped to the task template: 
\textbf{TEDL4: For a given $<reference\_set>X$, does the $<characteristic> C$ [exceed a threshold/ equal a specific value / fall within a specific range]?}
Which is an elementary direct lookup task (see Table A1). 

%The next step is to map the task components to their corresponding tokens in the template. 
The first $<reference\_set>$ occurrence in the template is mapped to ``period of months'' in both example tasks. For these tasks, it is safe to assign a temporal variable that contains admission time as the first variable in their variable lists.
Again a distribution across different months is targeted in both tasks. 
%These first pieces of information, in addition to the value assigned for $\textbf{granT}$ can lead us to understand 
%lead the TaskMapper algorithm to assign the admission time variable to the x-axis in a visualization. It also 
%that TASHA will assign a variable read from the database that describes admission time to the x-axis on a visualization and will aggregate this variable on a monthly scale.

The second token in the TEDL4 template is $<characteristic>C$ which maps to the variable that needs to be monitored over time (since this is a direct lookup task template, the outcome will always be a characteristic). In the first example, this variable is ``call-to-balloon time'' which is directly found in the database and in the second it is ``length of stay'' which is derived from a simple subtraction of two variables representing time of admission and time of discharge. 
%These two variables are quantitative, but before we append them to the variable lists of their corresponding tasks, we note that they are characteristics of the \textit{patient} referrer type.
%Therefore, the $\mathbf{granP}$ entry needs to be checked for granularity. 
%Since the granularity is at a monthly level, this tells us that a per-unit aggregate (e.g. count, average, etc.) needs to be used instead of the original value. 
%The choice of aggregate is enforced by the wording of the task. 
%Tasks that require average or median or some other descriptive statistic will specify that in their body. 
%If no aggregate is specified, we regard the task template, the role of the aggregated characteristic and its corresponding referrer in it.
These variables will be aggregated on a monthly scale. However, we noticed that when users ask criteria-matching questions like these, they do not specify a certain aggregate rule (e.g. count, average. median, etc.). 
These questions are simply stated as yes/no questions. Therefore, users were interested in observing patterns of record counts that met and ones that did not meet the criteria specified. 
Given this reasoning, we append a variable for the ``criteria'' and give it an aggregate ``count''. Unlike the count variables in examples T1 and T2, the count of the criteria-matching tasks does not just aim to show counts for a specific value (e.g. the value ``dead'' in T1). It typically aims to provide a distribution of the variation between records meeting and those that are not meeting the criteria. Therefore, we specify their target here as `distribution'' rather than ``value'', and we add a grouping variable ``match'' that separates calculations for records meeting/ non-meeting the criteria. 

We note, also, that in these examples the questions mention an additional piece of information before it moves to the last token (the square brackets in TEDL4). 
Namely,  “patients with STEMI/nSTEMI admission status” in the first example and “patients with cardiac diagnosis” in the second example. 
These additional pieces of information are adding further variables to the $<characteristic> C$ vector. 
Both examples include nominal variables that need to be aggregated with record ``count''. 
The targets for these tasks differ in that the first one sets a distribution between two levels of a nominal field ``STEMI/nSTEMI'',whereas the second one gives a specific value that needs to be tested ``cardiac patients''. 

At this point, the task T3 has the following feature vector: 
$\mathbf{variables}: [time, criterion, match, patientType]$, 
$\mathbf{aggregates}: [month, count, group, group]$,
$\mathbf{targets}: [distribution, distribution, distribution, distribution]$;
and task T4 has the following feature vector:
$\mathbf{variables}: [time, criterion, match, diagnosis]$, 
$\mathbf{aggregates}: [month, count, group, group]$,
$\mathbf{targets}: [distribution, distribution, distribution, value]$;
%TEHL3: For a given $<reference_set>X$, does the $<characteristic>C$ of $<reference\_subset>S$ meeting $<characteristic_criteria>CS1,...CSn [exceed a certain threshold, equal a specific value, fall within a specified range]?$  
%Note that this new task is labeled with the code TEHL which stands for “Template of Elementary Hybrid Lookup”. We consider this task a hybrid between direct and inverse lookup because it involves both: 
 % A direct lookup of the characteristic C, given a known $<reference_set>X$
  %An inverse lookup to identify $<reference_subset>S$ which meets the criteria set for characteristic(s) CS1,…, CSn. 
%Given this expanded form, it is now straightforward to map the remaining components of the task to the tokens, as follows: 
%The dissection so far results in the following variables the lists of each task:
%Ex1: Variables: [admission time, call-to-balloon, admission status]
%Ex2: Variables: [admission time, length of stay, diagnosis]

The variable types vector for both tasks is $[t, q, n, n]$. 
This information could be fed to an algorithm which would potentially map the t variable to the x-axis, the q variable to the y-axis and the n variable(s) to color(s) or other visual encoding. 
However, prior to seeking recommendations for visual encoding, TASHA performs further reassignment of variables, based on task sequences, which will be described in later sections. 
Although the task feature vectors developed so far are not the final form that will be fed to the visualization generation phase, they constitute a useful starting point. 
%This information, however is not enough to make more design decisions about the mark type and the corresponding visual elements. To make these decisions, we need to fill the missing information in the feature vectors of the tasks. At this point, the format of the template becomes useful in better understanding the population granularity and the target information for each task. The yes/no nature of the template question “does the…?” means the users are interested to have a nominal value in the display that tells them where in the data the question is answered as “yes” and where it is answered as “no”. This additional nominal value needs to be calculated for the reference set(s) selected so far at a level of granularity that is specified by the granP element of the task specification. For the two example tasks above, the users are interested to monitor these metrics at the unit level. Therefore, the <characteristic>C variable in our task specification is replaced with a count of occurrences in which it meets the criteria specified in the square brackets and where it doesn’t meet such criteria. 
%This results in the partial specification shown in Figure~\ref{fig:grammar}[TODO: update this figure with the new task speci].



==> tex/grammar.tex <==
At this point in our task analysis, tasks are arranged in a master-slave manner in which a master is a task that has been selected by workshop participants as the most encompassing for a given metric. 
For example, when investigating delays in cardiology services, users are interested to answer the quality monitoring question: 
\textit{“Does the call-to-balloon time for STEMI patients meet the national target?” }
Slave tasks collected for this master include: 
\begin{itemize}
\item \textit{Were similar delays experienced for nSTEMI patients?}
\item \textit{Which of the delayed patients were direct/indirect admission?}
\item \textit{Which of the delayed patients were male/female?}
\item \textit{Were any of the delayed patients self-presented and did they commute a long distance? }
\item \textit{Should some records be excluded (e.g. because they are not patients of own hospital and experienced delays in referring hospital)?}
\end{itemize}
Note that for these slave tasks, the assumption is that the user is able to answer the master task first and identify references (i.e. times and patient groups) for which the target was not met. For more examples, please see Appendix B of the supplementary material. 

This two-step sequence provides some structure to guide the thinking process of a dashboard designer but not enough structure to automate parts of the design process. 
In this section, we describe a task grammar that expands upon the three-dimensional task space that was presented in~\cite{BELIV}. 
This grammar aims to replace a task specified in natural language with a more specific task feature vector, which in turn can be mapped to visualization attributes. 
Figure~\ref{fig:grammar} provides an example of the grammar components that describe a task [TODO: Not currently shown in this version of the figure]. 
%We note here that these components are not readily available in the responses collected from workshop participants. 
%In this Section, we describe the different components and demonstrate ones that could be directly elicited from participant responses. 

\begin{figure}[tb]
 \centering 
 \includegraphics[width=\columnwidth]{grammar.PNG}
 \caption{Grammar components to describe a task, based on the three-dimensional task space presented in~\cite{BELIV}.[TODO: modify this figure]}
 \label{fig:grammar}
\end{figure}


%Users would like to see a trend over time for the proportion of patients not meeting the target to the total number of admissions, and the proportion of those patients not meeting the target who are STEMI patients. Therefore, a target vector for this task is [“trend”, “proportion”, “proportion”].

\subsubsection{Expanding the Grammar for Task Sequences}

Having positioned the master in the task space, we then list all  tasks pertaining to this metric as children to the master task. 
To guide the choice of variable combinations to be fed to a visualization, we distinguish among three different types of relationships between a master and a slave task: 
\begin{itemize}
	\item $\mathbf{ISA}$: means the child task is part of a decomposition of the master task. This typically means that the set of variables involved in the child task are a subset of the variables involved in its parent. For example, the task “Which of the delayed patients were nSTEMI?” involves the same grouping variable that separates STEMI and nSTEMI patients in the master task. 
	\item $\mathbf{Extends}$: means the child task adds more variables to the mix. It builds upon what has already been identified in the master task and adds more variables that are used in a zoom-and-filter manner or to give details-on-demand. Examples for this type of tasks include: 
	Which of the delayed patients were direct/indirect?
	Which of the delayed patients were male/female?
	Which of the delayed patients were self-presented and commuted a long distance? 
	\item $\mathbf{Alters}$: means the child task provides other alternative hypotheses that can either entirely substitute the master task or modify the data shown for it. An example of this type of task is: “Should some records be excluded (e.g. because they are not patients of own hospital and experienced delays in referring hospital)?” 
\end{itemize}

Each slave task gets positioned in the 3D task space by specifying its granularity (time and population), type cardinality and target(s). 


==> tex/method.tex <==

%\textcolor{green}{READY FOR COMMENTS}

We followed the design study methodology by Sedlmair et al.~\cite{sedlmair2012design} to introduce visualization dashboards for national clinical audit data in five NHS hospitals. 
This section outlines the activities we performed in each of the four stages in the core phase of the methodology. 
In the \textit{Discover} stage we analyzed qualitative data that we collected through interviews with 54 healthcare professionals of various backgrounds.
We used this data to build a thematic understanding of organization-level \texttt{metrics} which set unique requirements for individual audits. For each metric, we collated queries and quotes from the interview transcripts that led to the generation of an initial set of tasks. Section~\ref{sub:gen} describes the details of this task generation phase. 
%To avoid such pitfalls as ignoring working practices and focusing only on a subset of measures (tunnel vision~\cite{chearskul2010empirical}), we asked ourselves the question: Can a taxonomic approach be beneficial to the problem characterization and abstraction stage of dashboard design? This question was motivated by the argument made by Kerracher et al.~\cite{kerracher2017constructing} that by setting out the range of potential tasks of interest (i.e. the task space), one may overcome known problems associated with simply asking people to introspect.
%It was also motivated by models like Draco which sought to formalize and incorporate user tasks in the process of visualization authoring~\cite{moritz2019formalizing}.

We organized two co-design workshops in which groups of stakeholders participated. The purpose of the co-design activities was to capture a broad coverage of the task space, task sequences and design alternatives. 
Rather than considering each task as a standalone knowledge construct,
we were inspired by the Brehmer and Munzner Typology (BMT)~\cite{brehmer2013multi} to elicit contextual information that helped us connect tasks in sequences based on contexts of use (the \textit{why}), visualizations used in current practice (the \textit{how}) and input and output for each task (the \textit{what}). 
%Furthermore, We elicited participant's sketches to inform these connections and understand users' expectations/vision of the dashboard. 
Section~\ref{sub:task} details the workshop material and procedure, then summarizes the requirements for the QualDash software based on findings from the interviews and workshops. 

For the \textit{Design} stage, 
%In the \textit{Implement} stage,
we describe a novel semi-automated dashboard generation engine in Section~\ref{sec:design}. 
We developed this engine to provide dashboard authoring capability at the organization level, while allowing a limited set of customization interactions for individual end users. 
Specifically, we define a visual construct called the \texttt{metric card}, which acts as a building block for dashboard generation and adaptation. 
Each metric card is designed to cater to the visualization needs of a specific healthcare quality metric, and is generated from a JSON specification structure, which we refer to in the remainder of this paper as the Metric Specification Structure (MSS). 
The dashboard engine accepts an array of MSSs and generates the corresponding number of metric cards. 
%The MSSs are inspired by the Vega-Lite grammar~\cite{satyanarayan2017vega}, and represent a two-step hierarchy of patterns (Figure~\ref{fig:flow}(E)) that match the two-step task hierarchy (Figure~\ref{fig:flow}(D)).
%The MSSs are fed to the dashboard engine in the form of JSON structures, which are then used to generate the corresponding \textit{metric cards} on the dashboard (Figure~\ref{fig:flow}(e)). 
Section~\ref{sub:spec} describes the key-value elements that make up the MSS, based on the requirements identified in Section~\ref{sec:require}.
Next, we explain how the MSSs inform the dashboard generation and reflect on design decisions in Section~\ref{sub:card}. 

In the \textit{Deploy} stage, we describe feedback we  collected over the course of six months through 62 hours of on-site meetings with IT professionals and dashboard stakeholders. 
%The first meeting took the form of a two-session workshop involving participants from one hospital.
%The first session featured active intervention with a paper prototype, and in the second session we asked participants to interact with the dashboards and practice a think-aloud protocol. 
%These interactions were video-recorded and analyzed.
%video-recorded this latter session to ensure that all interactions with the dashboard and their thinking process is taken into account. 
Analyzing and addressing feedback was inspired by Lloyd and Dykes~\cite{lloyd}. Namely, we broke down comments into four categories: data-related, interface-related, interaction-related and new-related. We then found a need to further subdivide the interface-related category into: GUI-related and visualization-related. This distinction was important to prioritize visualization-related feedback that had a direct impact on data understanding and decision making. 
%In subsequent focus group meetings, feedback was elicited from stakeholders in the other hospitals and was added to the corresponding feedback category. 
We took the software into a final development iteration to address the prioritized feedback items.
Section~\ref{sec:valid} describes this evaluation phase of the project and Section~\ref{sec:conc} concludes our work. 


==> tex/metriccard.tex <==
 Originally developed by Kaplan and Norton, BCS's were introduced as \textit{``as an approach to integrating financial and non-financial measures into
management in the hyper-competitive environment''}~\cite{kaplan1992}.
 A typical scorecard includes at least four perspectives (financial, customers, internal
processes, and learning and growth) for each of which the organisation identifies a
number of goals and measures for gauging the degree of target attainment~\cite{assiri2006profit}.
This two-step hierarchy between \textit{perspectives} and \textit{measures} maps to the two-step hierarchy identified in our task analysis of \textit{master} and \textit{slave} tasks, where a master task typically overviews a metric ($\approx$a perspective) and the slave tasks examine different measures that pertain to the metric.  

Similar to the BSC which typically uses proximity to group measurements and enclosure/ closure to group perspectives~\cite{pover}, we first introduced to our stakeholders the idea of a Metric Bubble, which was inspired by Code Bubbles~\cite{bragdon2010code} and VisBubbles~\cite{li2011visbubbles}, as an enclosed view that allows flexible and adaptable dragging and resizing.
We felt that this adaptability would allow users to prioritize specific metrics and dedicate more prevalent areas of the screen to visualizations pertaining to those metrics. 
The idea of enclosure for metric-related tasks in one bubble was well-received. However, the free dragging and resizing behaviour for the bubbles was perceived as overwhelming and allowing \textit{``too many alternatives''} by three of our domain experts. 
They argued for a more restricted mechanism for laying out and resizing the metric enclosures on the screen. 
To accommodate this feedback, we considered two options for the layout: a tabbed view would display each metric enclosure on an individual tab, and a grid layout would place them on a single screen in a tiled manner. 
We chose the latter design alternative for two reasons: 
(a) the tabbed view misses out on the advantage of the BSC in that it integrates different perspectives in \textit{one consolidated viewpoint}, and (b) empirical evidence shows that juxtaposed
patches on a grid layout significantly reduced navigation mistakes over tabbed views~\cite{henley2017toward}. Despite that this finding was reported for code editors, we believe that the transition between examining different code fragments has some cognitive similarity to the process of proceeding from one metric to another. 

\begin{figure}[tb]
 \centering 
 \includegraphics[width=.9\linewidth]{pictures/dashMain.PNG}
 \caption{Main dashboard view for the PICANet audit showing 6 metric cards in their non-expanded form.} 
 %TODO: Scan these for better image quality
 \label{fig:dashMain}
\end{figure}

Figure~\ref{fig:dashMain} shows the main dashboard view for the PICANet audit. Six metric cards were generated from 6 Metric Specification Structures (MSSs) described in Section~\ref{sub:mss}. The cards are generated dynamically so adding a card is as simple as adding an additional MSS to the array describing the dashboard. 
Once specified, the metric card in its original form will display a visualization in either a single or trellis view depending on the number of measures that need to be monitored for each metric. Design choices made for each visualization are discussed in detail in Section~\ref{sub:choices}. For now, we highlight the correspondence between this regular grid view (Figure~\ref{fig:dashMain}) and the expectations set by our participants in the codesign activity shown in Figure~\ref{fig:activ2} (a) and (b). 

Adapting the initial dashboard layout is done by dragging the metric cards. This dragging behaviour is restricted to simulate a card shuffle behaviour, i.e. dragging one card will shuffle the positions of other cards to maintain the grid. The forces between cards are maintained by Muuri.js and the cards are implemented in HTML. 
Resizing a card is performed by double clicking the card. Once performed, the card toggles between its original form (shown in Figure~\ref{fig:dashMain}) and an expanded form (shown in Figure~\ref{fig:expand}). 
In the original form, the visualizations included in the card only address the master task of the card's corresponding metric; whereas in the expanded form more views are added to support the inclusion of additional variables. These additional variables are determined by the referrers and characteristics involved in the slave tasks for the metric. 
Views within a metric card are linked to enable composite brushing and linking. However, we avoid cross-card interaction to reflect the nature of our task space, in which tasks pertaining to different metrics are self-contained and have very little interaction with other metrics. 
This idea of self-contained cards also addresses comments made by clinicians in our co-design participants group, in which they noted that once they focus on examining a metric, other metrics become peripheral to their thinking process. 
This may not be the case in other applications.
We note there that by introducing the metric card metaphor, we define an intermediate level of layout grouping between the single visualization view and the dashboard. This intermediate level offers a lot of flexibility and adaptability and introduces the area of dashboard design to a number of new possibilities to 
use connection, continuity, and similarity to assemble cause-effect and cascading relationships across cards.

\begin{figure*}[tb]
 \centering 
 \includegraphics[width=.9\linewidth]{pictures/change_vars.png}
 \caption{Dashboard view for the PICANet audit showing one expanded metric card and two non-expanded cards in the periphery.} 
 %TODO: Scan these for better image quality
 \label{fig:expand}
\end{figure*}

==> tex/overview.tex <==

\textcolor{green}{READY FOR COMMENTS}

The TASHA workflow extends the core phase of the design study methodology by Sedlmair et al.~\cite{sedlmair2012design}.
Our workflow links together contributions in each of the four stages in the core phase of the methodology: \textit{Discover}, \textit{Design}, \textit{Implement} and \textit{Deploy}.
Specifically, we describe a five-stage typology-driven workflow to design, implement and evaluate an adaptable quality dashboard tool to be deployed in five NHS Hospitals. 

\bstart{In the \textit{Discover} stage} we analyzed qualitative data that we collected through interviews with 54 healthcare professionals of various backgrounds.
We transformed this data into a structural understanding of the department-level goals and measures which set unique requirements for every individual dashboard.
%To avoid such pitfalls as ignoring working practices and focusing only on a subset of measures (tunnel vision~\cite{chearskul2010empirical}), we asked ourselves the question: Can a taxonomic approach be beneficial to the problem characterization and abstraction stage of dashboard design? This question was motivated by the argument made by Kerracher et al.~\cite{kerracher2017constructing} that by setting out the range of potential tasks of interest (i.e. the task space), one may overcome known problems associated with simply asking people to introspect.
%It was also motivated by models like Draco which sought to formalize and incorporate user tasks in the process of visualization authoring~\cite{moritz2019formalizing}.
The first three stages of the TASHA framework aim to formalize the interview-collected tasks in a way that enables the reduction of the task space to a manageable size, which can be taken further into the design stage  (Figure~\ref{fig:flow}(a) and (b)). 
%This reduction process is done systematically to maintain coverage and avoid skewing the space toward a particular user group while ignoring others. 
In Section~\ref{sec:tschar} we describe the first level of the mapping from raw natural language task descriptions to clusters of task features, based on the AA Task Typology~\cite{andrienko2006exploratory}. 
Section~\ref{sub:data} describes the raw interview data along with a description of the data model of National Clinical Audit databases, which underlie the development of the dashboard tool.
In Section~\ref{sub:dissect}, we extend the AA Typology to dissect each task and understand its skeletal features. 
As a result of this understanding, we explain the task clusters we identified and our sampling strategy to select one representative task from each cluster in Section~\ref{sec:sampling}. 
%The purpose of this selection process is to reduce the task space to a manageable size which can then be used in co-design activities. 

%We then used the AA Task Typology~\cite{andrienko2006exploratory} to understand the skeletal structure of each one of these questions, and obtain task clusters based on this undertanding. 


\bstart{In the \textit{Design} stage}
we describe activities that we organized for a co-design workshop in which a group of stakeholders participated (Figure~\ref{fig:flow}(c)). The purpose of the activities was to obtain a bigger picture on the task space: rather than considering each task as a standalone knowledge construct. 
Inspired by the Brehmer and Munzner Typology (BMT)~\cite{brehmer2013multi}, we elicited contextual information that would help us
connect the tasks in sequences based on context of use (the \textit{why}), visualizations used in current practice (the \textit{how}) and input and output for each task (the \textit{what}). 
We elicited participant's sketches to inform these connections and understand users' expectations/vision of the dashboard. 
Section~\ref{sec:sequencing} details the workshop material (Section~\ref{sub:material}) and procedure (Section~\ref{sub:proc}), then summarizes results and findings of the workshop (Section~\ref{sub:wres}). 

\bstart{In the \textit{Implement} stage}
we describe a novel semi-automated dashboard generation engine in Section~\ref{sec:spec}. 
We developed this engine to provide dashboard adaptation capability to a small group of users (the dashboard authors), while allowing a limited set of customization options open to all end users. 
Specifically, we mapped the task sequences for two different dashboards to a set of metric specification structures (MSSs).
This mapping was reviewed in meetings with three domain experts to ensure its validity.
%The MSSs are inspired by the Vega-Lite grammar~\cite{satyanarayan2017vega}, and represent a two-step hierarchy of patterns (Figure~\ref{fig:flow}(E)) that match the two-step task hierarchy (Figure~\ref{fig:flow}(D)).
The MSSs are fed to the dashboard engine in the form of JSON structures, which are then used to generate the corresponding \textit{metric cards} on the dashboard (Figure~\ref{fig:flow}(e)). 
Section~\ref{sec:spec} describes the parsing of task sequences into JSON structures, 
First, we explain the metric card metaphor as a self-contained area of the dashboard in
Section~\ref{sub:metriccard}. Then we define the mapping from task sequences to MSSs in Section~\ref{sub:mss}.  
Finally, we explain how the MSSs inform the view generation and reflect on design decisions in Section~\ref{sub:choices}. 


\bstart{In the \textit{Deploy} stage} we describe feedback we have collected over the course of five weeks through a number of focus group meetings with stakeholders from the five hospitals. 
The first meeting took the form of a two-session workshop involving participants from one hospital.
The first session featured active intervention with a paper prototype, and in the second session we asked participants to interact with the dashboards and practice a think-aloud protocol. 
These interactions were video-recorded and analyzed.
%video-recorded this latter session to ensure that all interactions with the dashboard and their thinking process is taken into account. 
Analyzing the results of both sessions was inspired by Lloyd and Dykes~\cite{lloyd}. Namely, we broke down feedback into four categories: data-related, interface-related, interaction-related and new-related. We then found a need to further subdivide the interface-related category into: GUI-related and visualization-related. This distinction was important to prioritize visualization-related feedback that had a direct impact on data understanding and decision making. 
In subsequent focus group meetings, feedback was elicited from stakeholders in the other hospitals and was added to the corresponding feedback category. 
We then took the software into a final development iteration to address the prioritized feedback items.
Section~\ref{sec:valid} describes this evaluation phase of the project and Section~\ref{sec:conc} concludes our work. 


==> tex/trash.tex <==
Despite the variability of tasks and designs collected through our co-design processes, some common threads exist. For example, most of the designs provided by participants included one or more bar charts to monitor measurements over time. When asked about their choice of bar chart rather than a line chart or scatter plot, participants agreed that bar charts are more intuitive than the other alternatives. One expert noted \textit{``If I see a bar chart while passing by my computer screen, I can immediately spot if there is a spike or something unusual, but if you show me a scatter plot I will bring my glasses, sit with my coffee and look at the visualization for a while before I'd understand what is going on''}.
This and similar arguments made by participants motivated the choice of bar chart variants for the main metric view. 


\begin{table*}
	\caption{List of tasks pertaining to the Mortality Metric}
	\label{tab:mort}
	\centering
	\scriptsize
	\resizebox{0.9\textwidth}{!}{%
	\begin{tabular}{|c|l|c|c|c|c|}
		\hline
		 \textbf{Code} & \textbf{Task} & Q & N & O & T \\
		\hline
		\hline
		${TM}^{\ast}$ & \textbf{Master:} What is the trend of admissions and inpatient mortality per month? [SBC1] & 2 & & & 1 \\
		\hline
		& \textbf{Slaves:} &  & & &  \\
		$TM1$&	\multicolumn{1}{|l|}{\textbullet On a month with high mortality, did patients come straight or from another hospital? [SBC5] } &  & + 1 & &  \\
	    $TM2$ & \multicolumn{1}{|l|}{\textbullet For deceased patients, what was the reason of admission? [SBC5] } &  & + 1 & &  \\
		$TM3$ & \multicolumn{1}{|l|}{\textbullet Were patients of a specific gender or ethnicity more likely to die? [SRS] } &  & + 1 & &  \\
		$TM4$ & \multicolumn{1}{|l|}{\textbullet For deceased patients on a given month, does a pattern exist in length of stay? [SBC6] } & + 1  & & &  \\
		$TM5$ & \multicolumn{1}{|l|}{\textbullet On a month with high mortality, what was the average length of stay? [SBC5] } & + 1 &  & &  \\
	    %$TM5$ & \multicolumn{1}{|l|}{\textbullet Are the majority of patients leaving the hospital alive or dead? [SBC6] } & + 1  &  & & \\
		$TM6$ & \multicolumn{1}{|l|}{\textbullet What time interval has a considerable rise in mortality (months, quarters, years)? [SRS] } &  & & & + 2 \\
		$TM7$ & \multicolumn{1}{|l|}{\textbullet How does admission on a monthly basis compare to previous years? 
		? [SCOM] } &  &  & & + 1 \\
		\hline
	\end{tabular}
	}
\end{table*}


%Participants opted to use different ways to sketch the life cycle of a task. 
%Figure~\ref{fig:activ1} shows three examples: in \textit{(a)} participants explained that in order to decide whether or not delays in care delivery were justified (Task $T37$ in Table S1), 
%In \textit{(b)} we show a new task that was added by participants:  \textit{``Is the Trust an outlier nationally or compared to peer trusts?''}
%They explained (with sketches) that this high-level question contextualizes several other tasks. For example, it encapsulates an understanding of the monthly mortality rates ($T1$), age group distribution ($T5$), length of stay ($T17$), admission method ($T30$), etc. It also leads to new questions about the data quality, patient pathways, etc. 
In the example shown in Figure~\ref{fig:activ1}\textit{(c)} another user-crafted task asked about data completeness. To contextualize this task, the participant chose to sketch a flow diagram showing the data journey for the MINAP audit and noted the most important variables that are typically looked at when answering this question. 

\bstart{Task sequences}
Links between tasks that were identified through the first activity offered an understanding of their contextual groupings. Think of these task groups as a set of disconnected subgraphs where the nodes represent the tasks and the links depict the relationships among them. 
Task sequencing then aimed at identifying whether this graph is a directed one, i.e. whether there exists a specific order in which these groups of tasks are performed. 

 By examining the sketches (Figure~\ref{fig:activ2}), it was clear that participants organized these entry-point tasks around a set of unique metrics for each audit, and that for each metric, the dashboard was expected to start with a minimalist representation that either simply lists the names of the variables involved (e.g. Figure~\ref{fig:activ2}(a)) or answered a short question about each metric (e.g. Figure~\ref{fig:activ2}(b)) by use of simple visualizations involving up to two referrers and up to six characteristics (e.g. Figure~\ref{fig:activ2}(c)). 

Participants then added some of the remaining tasks that were collected through the first activity, in an extended part of their sketches (Figure~\ref{fig:activ2}(c)) and highlighted that they expected these additional views to be added upon interacting with the software. One group agreed that it would be good to \textit{``double-click to see more''} as a way to proceed from the initial view of each metric. 
 The next step in our analysis was to connect these Entry-Point Tasks (EPTs) to their \textit{``children''} tasks. These are the tasks which would involve simple interactions (e.g. a double-click) to display their respective visualizations. 
We refer to this two-step sequence as a master-slave relationship in the remainder of this paper, where each metric has one EPT as a master and a number of slaves. 
This is to characterize the hierarchical nature of the relationship where a master task holds the key to answering its slave tasks, therefore needs to be addressed first. 

In analyzing the results of the workshop, we found it easiest to start with where the discussion had ended. Namely, we looked at the entry point tasks that were selected by participants and found that they all involve a combination of instances of the template form: 
\textbf{SBC1: What is the $<pattern>$ of $<characteristic\_1>$ of $<reference(s)\_of\_set\_1>$  [over/per] $<reference(s)\_of\_set\_2>$?}
 and that up to 7 such tasks needed to be answered simultaneously with zero-interaction for each audit's dashboard.







\begin{figure*}[tb]
 \centering 
    \subfloat[\label{left}]{
        \includegraphics[width=.3\linewidth, height=1.6in]{pictures/cquin_edited.jpg}
    }
    \hfill
    \subfloat[\label{center}]{
        \includegraphics[width=.3\linewidth, height=1.6in]{pictures/dashboard_edited.jpg}
    }
    \hfill
    \subfloat[\label{right}]{
        \includegraphics[width=.3\linewidth, height=1.6in]{pictures/julia_edited.jpg}
    }
 \caption{Identifying entry-point tasks (Activity 2).} 
 %TODO: Scan these for better image quality
 \label{fig:activ2}
\end{figure*}

\begin{figure*}[tb]
 \centering 
 \includegraphics[width=\linewidth]{pictures/results2.png}
 \caption{ Example breakdown of feedback from one of the focus group sessions: Session II - Think-aloud Protocol.} 
 %TODO: need better image quality?
 \label{fig:res}
\end{figure*}




\begin{table*}
	\caption{Results.}
	\label{tab:results}
	\centering
	\scriptsize
	\resizebox{\linewidth}{!}{%
	\begin{tabular}{c|c|c|c|c|c|c|c|c|}
	\cline{3-9}
	 \multicolumn{2}{ c| }{} & \multicolumn{6}{ c| }{Evaluation Method} & %\cellcolor{light-gray} 
	 \\
	 \cline{3-9}
	  \multicolumn{2}{ c| }{} & \cellcolor{light-gray} Paper Prototype & \cellcolor{light-gray} Think-aloud 1 &  \cellcolor{light-gray} Think-aloud 2 & \cellcolor{light-gray}Focus Group 1 & \cellcolor{light-gray}  Focus Group 2 & \cellcolor{light-gray} Focus Group 3 &  \cellcolor{light-gray} Total\\
	\cline{1-9}
	\multicolumn{1}{ |c  }{\multirow{2}{*}{Data-related} } & 
	\multicolumn{1}{ |c| }{$\mathbf{(+)}$} & 5 & 4 & 5 & 6 & 7  & 8 & 9 \\ 
	\cline{2-9}
	\multicolumn{1}{ |c  }{}  & 
	\multicolumn{1}{ |c| }{$\mathbf{(-)}$} & 2 & 4 & 5 & 6 & 7 & 8 & 9     \\ \cline{1-6}
	\cline{2-9}
	\multicolumn{1}{ |c  }{\multirow{2}{*}{Task-related} } & 
	\multicolumn{1}{ |c| }{$\mathbf{(+)}$} & 1 & 4 & 5 & 6 & 7  & 8 & 9 \\ 
	\cline{2-9}
	\multicolumn{1}{ |c  }{}  & 
	\multicolumn{1}{ |c| }{$\mathbf{(-)}$} & 2 & 4 & 5 & 6 & 7 & 8 & 9     \\ \cline{1-6}
	\cline{2-9}
	\multicolumn{1}{ |c  }{\multirow{2}{*}{Visualization-related} } & 
	\multicolumn{1}{ |c| }{$\mathbf{(+)}$} & 12 & 4 & 5 & 6 & 7  & 8 & 9 \\ 
	\cline{2-9}
	\multicolumn{1}{ |c  }{}  & 
	\multicolumn{1}{ |c| }{$\mathbf{(-)}$} & 3 & 4 & 5 & 6 & 7 & 8 & 9     \\ \cline{1-6}
	\cline{2-9}
	\multicolumn{1}{ |c  }{\multirow{2}{*}{Interaction-related} } & \multicolumn{1}{ |c| }{$\mathbf{(+)}$} & 0 & 4 & 5 & 6 & 7  & 8 & 9 \\ 
	\cline{2-9}
	\multicolumn{1}{ |c  }{}  & 
	\multicolumn{1}{ |c| }{$\mathbf{(-)}$} & 1 & 4 & 5 & 6 & 7 & 8 & 9     \\ \cline{1-6}
	\cline{2-9}
	\multicolumn{1}{ |c  }{\multirow{2}{*}{GUI-related} } & 
	\multicolumn{1}{ |c| }{$\mathbf{(+)}$} & 3 & 4 & 5 & 6 & 7  & 8 & 9 \\ 
	\cline{2-9}
	\multicolumn{1}{ |c  }{}  & 
	\multicolumn{1}{ |c| }{$\mathbf{(-)}$} & 0 & 4 & 5 & 6 & 7 & 8 & 9     \\ \cline{1-6}
	\cline{2-9}
	\multicolumn{1}{ |c  }{\multirow{2}{*}{Other} } & 
	\multicolumn{1}{ |c| }{$\mathbf{(+)}$} & 0 & 4 & 5 & 6 & 7  & 8 & 9 \\ 
	\cline{2-9}
	\multicolumn{1}{ |c  }{}  & 
	\multicolumn{1}{ |c| }{$\mathbf{(-)}$} & 0 & 4 & 5 & 6 & 7 & 8 & 9     \\ \cline{1-6}
	\cline{2-9}
		\hline
	\end{tabular}
	}
\end{table*}
In this paper, we present a multi-stage framework to navigate the dashboard design space while making use of principles of co-design in the context of quality monitoring in healthcare. 
We reflect on our experience of designing, developing and evaluating a set of visualization dashboards to be used in five different hospitals for the purpose of monitoring their quality of care using two different data sources: the Paediatric Intensive Care Audit Network (PICANet) data, and the  Myocardial Ischaemia National Audit Project (MINAP) data. 
The diverse user population for the dashboards includes physicians, nurses, 
audit support staff,
managerial board members,
quality and safety staff, information staff among others.
This diversity complicates the task analysis stage of the design study methodology~\cite{} and motivates substantial qualitative data collection during the early stages of the design life cycle. 

During these early stages, interviews with prospective dashboard users reveal a large number of tasks that the dashboard is expected to support.
Our proposed framework aims to systematically map this unstructured set of tasks into a structured format that can then be fed into a dashboard generation engine. This direct mapping between tasks and visualization has many advantages including the construction of a mental model tha ...  




Dashboard design is often challenged by the heterogeneity of user tasks that need to be supported.


Qualitative techniques are proven to 

%% \section{Introduction} %for journal use above \firstsection{..} instead
Our contributions in this paper are: 
\begin{itemize}
    \item A two-step sequence of abstract user tasks, in the context of dashboard design
    \item A taxonomy-driven framework to systematically guide the processes of task specification and dashboard co-design
    \item A view specification data structure that enables the dynamic generation of dashboard views based on task features. 
\end{itemize}

\begin{itemize}
\item \textbf{BC1: What is the $<\textcolor{blue}{pattern}>$ of $<\textcolor{blue}{characteristic\_1}>$ of \\ $<\textcolor{blue}{reference(s)\_of\_set\_1}>$  [over/per] \\ $<\textcolor{blue}{reference(s)\_of\_set\_2}>$?}
    
\item \textbf{BC2: On a given $<\textcolor{blue}{association\_pattern}>$ of $<\textcolor{blue}{characteristic\_1}>$ in $<\textcolor{blue}{reference(s)\_of\_set\_1}>$, what is the $<\textcolor{blue}{pattern}>$ of $<\textcolor{blue}{characteristic\_2}>$ of $<\textcolor{blue}{reference(s)\_of\_set\_2}>$ ? }
\begin{itemize}
    \item[] \textit{``T2: On a month with high mortality, what is the average length of stay?''}
        \begin{itemize}
        \item $<\textcolor{blue}{association\_pattern}> := high\_values$
        \item $<\textcolor{blue}{characteristic\_1}> := death$
        \item $<\textcolor{blue}{reference(s)\_of\_set\_1}> := patients$
        \item $<\textcolor{blue}{pattern}> = average$
        \item $<\textcolor{blue}{characteristic\_2}> := $ $length$ $of$ $stay$
        \item $<\textcolor{blue}{reference(s)\_in\_set\_2}> := months$
        \end{itemize}
    \end{itemize}
\end{itemize}


\begin{table}
	\caption{Mapping two example tasks to their corresponding templates}
	\label{tab:taxex}
	\centering
	\scriptsize
	\resizebox{\columnwidth}{!}{%
	\begin{tabular}{|c|c|c|c|}
		
		\hline
		 Audit & Elementary & Synoptic & Breakdown \\
		\hline
		PICANet &  &  & \multicolumn{1}{|l|}{\textbullet Behaviour characterization:} \\
		 & & & \multicolumn{1}{|l|}{\textbullet Pattern Search:} \\
		 & & & \multicolumn{1}{|l|}{\textbullet Comparison:} \\
		 & & & \multicolumn{1}{|l|}{\textbullet Relation seeking:} \\
		
		\hline
		MINAP & 1\% & 99\% & \multicolumn{1}{|l|}{\textbullet Behaviour characterization:} \\
		 & & & \multicolumn{1}{|l|}{\textbullet Pattern Search:} \\
		 & & & \multicolumn{1}{|l|}{\textbullet Comparison:} \\
		 & & & \multicolumn{1}{|l|}{\textbullet Relation seeking:} \\
		\hline
	\end{tabular}
	}
\end{table}

\begin{table*}
	\caption{Task-driven Metric Specification Structure (MSS) and corresponding Vega-Lite Grammar for the task(s) in Table~\ref{tab:mort}.}
	\label{tab:mss}
	\centering
	\scriptsize
	
	\begin{tabular}{|ll|}
		\hline
		
 \rowcolor{lighter} MSS example & Vega-Lite Example   \\
\hspace{2mm}\texttt{\{} & \hspace{2mm}\texttt{\{} \\
        \hspace{4mm} \texttt{"\textcolor{brown}{metric}": "Call-to-Balloon",} 
        & \hspace{4mm} \texttt{"\textcolor{brown}{data}": \{"\textcolor{brown}{url}": "minap.csv",} \\
         
         \hspace{4mm} \texttt{"\textcolor{brown}{mark}": "bar",} 
         & \hspace{4mm} \texttt{"\textcolor{brown}{mark}": "bar",} \\
         
         \hspace{4mm} \texttt{"\textcolor{brown}{x}": "bar",} 
         & \hspace{4mm} \texttt{"\textcolor{brown}{encoding}":  \{ } \\
         \hspace{4mm} \texttt{"\textcolor{brown}{mark}": "bar",} 
         & \hspace{4mm} \texttt{"\textcolor{brown}{mark}": "bar",} \\
         \hspace{4mm} \texttt{"\textcolor{brown}{mark}": "bar",} 
         & \hspace{4mm} \texttt{"\textcolor{brown}{mark}": "bar",} \\
         \hspace{4mm} \texttt{"\textcolor{brown}{mark}": "bar",} 
         & \hspace{4mm} \texttt{"\textcolor{brown}{mark}": "bar",} \\
         \hspace{4mm} \texttt{"\textcolor{brown}{mark}": "bar",} 
         & \hspace{4mm} \texttt{"\textcolor{brown}{mark}": "bar",} \\
         
\hspace{2mm}\texttt{\}} & \hspace{2mm}\texttt{\}} \\
		
		\hline
	\end{tabular}
	
\end{table*}

\begin{figure}[tb]
 \centering 
 \includegraphics[width=.9\linewidth]{pictures/json.png}
 \caption{Example Metric Specification Structure (MSS) for the mortality metric shown in Table~\ref{tab:mort}.} 
 %TODO: need better image quality
 \label{fig:json}
\end{figure}


